Formal Specification and Verification of Smart Contracts for Azure Blockchain

Ensuring correctness of smart contracts is paramount to ensuring trust in blockchain-based systems. This paper studies the safety and security of smart contracts in the \emph{Azure Blockchain Workbench}, an enterprise Blockchain-as-a-Service offering from Microsoft. As part of this study, we formalize \emph{semantic conformance} of smart contracts against a state machine model with access-control policy and develop a highly-automated formal verifier for Solidity that can produce proofs as well as counterexamples. We have applied our verifier {\sc VeriSol} to analyze {\it all} contracts shipped with the Azure Blockchain Workbench, which includes application samples as well as a governance contract for Proof of Authority (PoA). We have found previously unknown bugs in these published smart contracts. After fixing these bugs, {\sc VeriSol} was able to successfully perform full verification for all of these contracts.

==> expts.tex <==
\section{Results}
\label{sec:results}

\newcommand{\AssetTransfer}{\texttt{AssetTransfer}}
\newcommand{\BasicProvenance}{\texttt{BasicProvenance}}
\newcommand{\BazaarItem}{\texttt{BazaarItemListing}}
\newcommand{\DefectiveComponent}{\texttt{DefectiveComponent}}
\newcommand{\DigitalLocker}{\texttt{DigitalLocker}}
\newcommand{\FreqFlyer}{\texttt{FrequentFlyer}}
\newcommand{\HelloBlockchain}{\texttt{HelloBlockchain}}
\newcommand{\RefrigeratedTrans}{\texttt{RefrigSupport}}
\newcommand{\RoomThermostat}{\texttt{RoomThermostat}}
\newcommand{\SimpleMarket}{\texttt{SimpleMarketplace}}

In this Section, we detail the use of \verisol{} on smart contracts present in the Azure Blockchain content and samples on github~\cite{workbench-samples}\footnote{As of commit \texttt{1571029} on August 7th, 2018.}.
In Section~\ref{sec:verisol-workbench}, we  describe the application to 8 Workbench sample contracts to check semantic conformance with respect to their state machine based Workbench Application Configuration (Section~\ref{sec:conformance}).
Next, in Section~\ref{sec:verisol-poa} we describe the application to check safety properties for the contracts for PoA governance.
We describe previously unknown bugs that have been found, confirmed and fixed by the authors of these contracts, and also report on unbounded verification for Workbench samples with respect to their specifications.

\vspace{5pt}
\noindent \textbf{Experimental Setup.}
All experiments were run on a Intel Xeon 3.6HGz machine with 32 GB RAM running Windows 10.

% high level summary
% details of each workbench sample
% LOC for each sample
% bugs found
% unbounded verification -- observation
% show invariant for AssetTransfer
% properties for poa
% bugs found -- assert/require, finalize, injected
% runtime for different bounds

\subsection{Workbench Samples}
\label{sec:verisol-workbench}

\vspace{5pt}
\noindent \textbf{Benchmarks.}

\vspace{5pt}
\noindent \textbf{Main Results.}

\vspace{5pt}
\noindent \textbf{Bugs found.}

%\begin{table*}[t]
%\begin{small}
%\begin{tabular}{cccccccccc}
%\hline
%\multirow{2}{*}{\bf Source} & 
%\multirow{2}{*}{\bf Contract} &
%\multirow{2}{*}{\bf LOC} &  
%\multirow{2}{*}{\bf Property} & 
%\multicolumn{5}{c}{\bf Time for Bound (secs)} &
%\multirow{2}{*}{\bf Time for } \\
%& & & & 1 & 2 & 4 & 8 & 16 & {\bf Unbounded} \\
%\hline
%Workbench & \AssetTransfer & & &  &  &  & & \\
%Workbench & \BasicProvenance & & &  &  &  & & \\
%Workbench & \BazaarItem & & &  &  &  & & \\
%Workbench & \DefectiveComponent & & &  &  &  & & \\ 
%Workbench & \DigitalLocker & & &  &  &  & & \\
%Workbench & \FreqFlyer & & &  &  &  & & \\
%Workbench & \HelloBlockchain & & &  &  &  & & \\
%Workbench & \RefrigeratedTrans & & &  &  &  & & \\
%Workbench & \RoomThermostat & & &  &  &  & & \\
%Workbench & \SimpleMarket & & &  &  &  & & \\
%\hline 
%PoA & & & Pr1 &  &  &  & & \\
%PoA & & & Pr2 &  &  &  & & \\
%PoA & & & Pr3 &  &  &  & & \\
%PoA & & & Pr4 &  &  &  & & \\
%\hline
%\end{tabular}
%\end{small}
%\caption{Bounded and unbounded verification of smart contracts, after any fixes applied.}
%\end{table*}


\begin{table}[t]
\begin{small}
\begin{tabular}{|c|l|}
\hline
{\bf Example} 
&  {\bf Description of workflow} \\
%& {\bf LOC}   \\
\hline
\AssetTransfer &  Selling high-value assets  \\
\BasicProvenance & Simple record of ownership  \\
\BazaarItem & Multiple workflow scenario for \\
            & selling items \\
%\DefectiveComponent & Fixed-length array of integers & \\
\DigitalLocker & Sharing digitally locked files  \\
%\FreqFlyer & Dynamic-length array of integers & \\
\HelloBlockchain & Request and response (Figure~\ref{fig:helloblockchain-fig})  \\
\RefrigeratedTrans & Provenance scenario with IoT \\
                   & monitoring  \\
\RoomThermostat & Thermostat installation and use  \\
\SimpleMarket & Owner and buyer transaction \\
\hline
\end{tabular}
\end{small}
\caption{Description of Workbench Samples.}
\label{tab:samples}
\end{table}

Table~\ref{tab:samples} summarizes the eight sample smart contracts that are offered as part of the Azure Blockchain Workbench.
%Workbench customers use these templates as a starting point to build more sophisticated workflows. 
We have already described one of the samples $\helloBlockchain$ in detail as our running example in Section~\ref{sec:overview}.
The remaining examples similarly demonstrate some  customer scenario workflow.
For example, $\AssetTransfer$ is a workflow for selling a high-value asset such as a house that involves several parties such as a seller, buyers, inspector, appraisers etc. 
$\DigitalLocker$ illustrates a workflow for sharing a digitally locked file. 
$\RefrigeratedTrans$ demonstrates the integration of events from IoT temperature sensor devices to monitor if a refrigerated shipment has not gone bad.
For each of these samples, we use a utility tool \appEnforcer{} to instrument the Solidity code with checks for semantic conformance similar to that described in Section~\ref{sec:solidity-instrumentation}. 
The resulting Solidity program is fed to \verisol{} to verify the assertions. 

\subsubsection{Bugs Found}
\label{sec:workbench-bugs}

We report on three bugs that \verisol{} found in the sample, related to incorrect initial state and state transition.

\begin{figure*}[htbp]
\centering
\includegraphics[scale=0.55]{assettransfer-config.PNG}
\caption{\AssetTransfer{} access control and state transition specification.}
\label{fig:assettransfer-configuration}
\end{figure*}


\begin{figure}[htbp!]
\begin{lstlisting}[style=Sol]
function Accept() public
{
  if (msg.sender != InstanceBuyer && $\label{line:at-line1}$ 
      msg.sender != InstanceOwner) {
     revert();
  }
  ...
 
  if (msg.sender == InstanceBuyer) { $\label{line:at-line2}$ 
     ...
  }
  else {
     // msg.sender has to be InstanceOwner 
     // from the revert earlier 
     if (State == StateType.NotionalAcceptance) { $\label{line:at-line3}$ 
        State = StateType.SellerAccepted;
     }
     else if (State == StateType.BuyerAccepted) { $\label{line:at-line4}$ 
        // BUG: Should be StateType.SellerAccepted
        State = StateType.Accepted;         $\label{line:at-line5}$ 
     }
  }
  ...
}
\end{lstlisting}
\vspace{-0.1in}
\caption{Function \texttt{Accept} of \AssetTransfer.}
\label{fig:assettransfer-smart-contract}
\end{figure}

\paragraph{\bf \AssetTransfer.}
Figure~\ref{fig:assettransfer-configuration} provides a pictoral description of the the access control and state transitions for the contract \AssetTransfer{} \footnote{\url{https://github.com/Azure-Samples/blockchain/tree/master/blockchain-workbench/application-and-smart-contract-samples/asset-transfer}}. 
It is a fairly non-trivial state transition system where the actions are guarded by membership of \texttt{msg.sender} within one of the roles or instance role variables. 
\verisol{} found a bug where the transition from the state \texttt{BuyerAccepted} to \texttt{SellerAccepted} was incorrectly implemented in the accompanying smart contract.
The specification allows a transition between the two states when invoking the function \texttt{Accept} when \texttt{msg.sender} equals the instance role variable \texttt{InstanceOwner} (abbreviated as \texttt{IO} in the diagram).
However, the implementation of the function \texttt{Accept} in Solidity transitions to the state \texttt{Accepted} instead under the same transition. 
%Due to the bug, the state of the workflow in the GUI of Workbench and the actual state on the blockchain will diverge.
%The GUI state will transition to \texttt{SellerAccepted} whereas the blockchain state will transition to final state \texttt{Accepted}.
%As a result, the user will see multiple transitions enabled from the new GUI state (namely \texttt{RescindOffer} and \texttt{Accept}), however, the smart contract does not have any matching action given that it has reached the final state. 
%This will result in blockchain transactions to revert without informing the user of the potential livelock. 


This is an example of a fairly deep bug, as it requires at least 6 transactions to reach the state \texttt{BuyerAccepted} from the initial state, each executing a function with several lines of Solidity code.
We can speculate that the author of this sample either did not have tests that exercised such deep transactions, or test oracles to observe the incorrect transition. 
The defect trace is an interprocedural trace terminating with \texttt{Accept}.
The trace within \texttt{Accept} consists of lines~\ref{line:at-line1}, ~\ref{line:at-line2}, ~\ref{line:at-line3}, ~\ref{line:at-line4} and ~\ref{line:at-line5}.
The transaction bounded verification using \corral{} found this bug within 5.96 seconds.
In the process, it inlined 954 procedures indicating the non-trivial search required to discover the defect. 

\paragraph{\bf \DigitalLocker.}
\verisol{} found a bug related to incorrect initial state of the smart contract.
According to the specification, the start state of the contract should be \texttt{Requested}, however the constructor terminates in  \texttt{DocumentReview}.
This was confirmed as a true bug and was introduced while porting the smart contract and an older code, for which the initial state was indeed \texttt{DocumentReview}; the configuration was updated to the new initial state, however the smart contract initial state was not refreshed.

\paragraph{\bf \BazaarItem.} 
We also found a similar bug where the initial state of a nested contract was not set according to the one specified in the JSON specification. 
This is an interesting contract that consists of two separate contracts \texttt{BazaarItemListing} and \texttt{ItemListing}, where a function in the former creates an instance of the latter contract using dynamic allocation \texttt{new ItemListing(...)}.
The state of the newly created \texttt{ItemListing} contract was set using a later function call. 
The source of the bug was related to the semantics of the Workbench JSON configuration specification for the case of nested contract creation.
Our bug pointed the developers to the ambiguity of the specification and the semantics was resolved in favor of fixing the bug. 

All the three bugs have been confirmed by the developers of Azure Blockchain content and samples, and have been fixed in their internal repositories and their internal tests have been updated; some of the bugs (e.g. \BazaarItem) have been fixed for the external code on github, and others will be updated in one of their future releases\footnote{As of December 12, 2018}. 

\subsubsection{Unbounded Verification}
\label{sec:workbench-verification}

Although the \corral{} based transaction-bounded verification allows us to explore fairly deep into the state space of the contracts, it does not offer any guarantees about arbitrarily large number of transactions. 
Besides, for a correct program, the verification takes longer as the transaction-bound is increased.
For example, for the \AssetTransfer{} contract, verifying the fixed version for bounds 6, 8, 10, 12 take respectively 5, 29, 79, 184 seconds. 

Once we fix the bugs in the sample contracts, we use the \houdini{}-based unbounded verification for the contracts.
Recall that \houdini{} requires the user to specify a candidate set of predicates at different program points (procedure entry and exit, and loop heads). 
A good choice of predicates relies on the property under consideration.
For the semantic conformance checking, we observe that most invariants relate to the values of the instance role variables.
For example, the smart contract code for \texttt{Accept} in Figure~\ref{fig:assettransfer-smart-contract} relies on comparisons of \texttt{msg.sender} with various instance role variables such as \texttt{InstanceOwner} and \texttt{InstanceBuyer}.
Based on this observation, we generate a set of candidate predicates for the top-level loop in the harness \texttt{main} generated for a contract.
Since the only variables in scope at the loop head are the state variables, we consider all possible aliasing and non-aliasing predicates between state variables of instance role type. 
That is, if \varn{x} and \varn{y} are state variables of some role type, we generate the following set of candidate predicates \{\varn{x} == \varn{y}, \varn{x} != \varn{y}, \varn{x} == 0x0, \varn{x} != 0x0, \varn{y} == 0x0, \varn{y} != 0x0 \}.

With these candidate predicates, \houdini{} infers safe inductive invariant that is (i) established by the constructor, and (ii) preserved by the execution of any public function of the contract, and (iii) verifies all the assertions present in the Boogie programs. 
For all the sample contracts, the invariant inference takes in the order of few seconds. 
For the case of the \AssetTransfer{} smart contract, we infer the following safe inductive invariant:
\[
\begin{array}{cc}
(\texttt{this.InstanceOwner} \neq 0x0) & \wedge \\
(\texttt{this.InstanceOwner} \neq \texttt{this.InstanceBuyer}) & 
\end{array}
\]

\subsection{PoA Governance Contracts}
\label{sec:verisol-poa}

\input{poa}


\subsubsection{Verification}

In this section, we describe the application of \verisol{} to the PoA Governance contracts that we described earlier in Section~\ref{sec:poa-overview}.
For these contracts, we check the correctness of assertions already present in the contracts, as well as additional safety specifications.
We have applied the bounded verification to these properties and report several injected and previously unknown bugs.

Recall that the PoA governance smart contracts implement the Parity {\it ValidatorSet} interface for managing PoA networks.
The ValidatorSet has the following interface, where \texttt{getValidators} returns the current set of validators.
The event \texttt{Initiatechange} is issued to signal a desire to  change  the validator set, and a call to \texttt{finalizeChange} to persist the change. 
\begin{figure}[htbp!]
\begin{lstlisting}[style=Sol,numbers=none]
contract ValidatorSet {
  event InitiateChange(bytes32 indexed _parent_hash, 
                       address[] _new_set);
  function getValidators() constant 
           returns (address[] _validators);
  function finalizeChange();
}
\end{lstlisting}
\vspace{-0.1in}
\caption{Parity ValidatorSet interface.}
\label{fig:poa-validatorset-interface}
\end{figure}

In Figure~\ref{fig:poa-properties}, we describe the properties we check for these contracts.
\texttt{Pr1} states that the system should always have at least one admin present; the network is initialized with a single admin at bootstrapping.
In case this invariant does not hold, the entire network will enter into a livelock state where any subsequent transaction will revert. 
\texttt{Pr2} ensures that no validator becomes {\it orphaned}; if an admin is voted out of the system, then all the validators that belong to the admin should also be removed from the list of validators. 
The developer of the contract informed us that this was one of the known bug that existed in a prior version of the contract that had since been fixed.
\texttt{Pr3} ensures that a validator does not belong to multiple admins; it can lead to unexpected consequences for the governance protocol.
Next, recall that the \texttt{AdminSet} is a contract that exposes a set interface to perform constant time operations such as lookup; since Solidity does not permit enumerating all the keys in a mapping, the set is implemented as a combination of an array of members \texttt{addressList} and a Boolean mapping \texttt{inSet} to map the members to true.
\texttt{Pr4} checks the coupling between these two data structures --- (i) \texttt{addressList} has no repeated elements, (ii) $\texttt{inSet}[a]$ is true if an only if there is an index $j$ such that  $\texttt{addressList}[j] == a$.
For the purpose of verification, we introduced a ghost variable that maintains the index $j$ into \texttt{addressList} for an address $a$.
Finally, \texttt{Pr5} checks that a call to a helper method \texttt{deleteArrayElement} is only invoked with an element present in the array; this is one of the assertions present in the original contract.
Most of the properties except \texttt{Pr4} require reasoning over all the contracts; \texttt{Pr4} requires reasoning about \texttt{AdminSet} and \texttt{Admin} contracts only, as it checks the set abstraction exposed by the \texttt{AdminSet} contract. 

\begin{figure}[!h]
\[
\begin{array}{|c|c|}
\hline
{\bf Property}  & {\bf Description}  \\\hline
{\tt Pr1}  & \textrm{There is at least one elected admin}  \\\hline
{\tt Pr2}   & \textrm{Every validator belongs to an elected admin}   \\\hline
{\tt Pr3}   & \textrm{No validator belongs to two elected admins}  \\\hline
{\tt Pr4}   & \textrm{AdminSet implements a set} \\\hline
{\tt Pr5}   & \textrm{\texttt{deleteArrayElement} deletes an element} \\\hline
%%...   & \textrm{...} \\\hline
\end{array}
\]
\caption{Properties for PoA governance contracts.}
\label{fig:poa-properties}
\end{figure}


\subsubsection{Bugs Found}
\label{sec:poa-bugs}

We now describe some of bugs that we found using the bounded verifier:

\paragraph{\bf \texttt{Pr5}.} 
We describe a sequence of transactions that results in  violation of this property.
The user issues a transaction to create an instance of \texttt{AdminValidatorSet}.
Let $x$ be one of the validators that are added for the first admin (say \texttt{admin0}) at the bootstrapping time. 
The \texttt{admin0} issues a transaction to remove the validator $x$ from its list of validators that results in a call to emit \texttt{InitiateChange} event after removing $x$ (using \texttt{deleteArrayElement}) from a internal validator set called \texttt{pendingValidatorSet}; a call to \texttt{finalizeChange} would persist this change. 
However, if \texttt{admin0} issues another transaction to remove $x$, then the call to \texttt{deleteArrayElement} fails the \texttt{Pr5} invariant, since $x$ has already been removed from the \texttt{pendingValidatorSet}.
Although this particular defect results in reverting certain (illegal) transactions, the scenario can be extrapolated to other buggy scenarios where an admin fails to add validators to the network. 
The bug resulted from a missing modifier that disallows two consecutive calls to \texttt{InitiateChange} without an call to \texttt{finalizeChange}.

\paragraph{\bf Assert as require.} 
\verisol{} was able to find counterexamples to several Solidity \texttt{assert} in the code that were actually meant to check for certain preconditions.
Although both \texttt{require} and \texttt{assert} failures revert an execution, Solidity  recommends using \texttt{assert} only for violations of internal invariants that are not expected to fail at runtime. 
Most of them could have been spotted during a code review as they were present in the first few lines of a public function; most of them checked for access control or avoid adding a duplicate validator or admin already present in the system by performing a lookup in a mapping.
However, there were a few asserts that were deeply nested inside private methods and relied on finding an element in an array (e.g. finding if a validator that is a candidate for removal is present in an array in an internal method \texttt{removeValidatorsInternal}). 

We note that these previously unknown defects in PoA contracts  only lead to safety violations, and as far as we could see, do not lead to security issues that can be exploited by a malicious user.
 
\paragraph{\bf Injected bugs}
In addition to the bugs above, we were able to use \verisol{} to find bugs that existed in prior versions of the contracts.
For example, we found a counterexample to \texttt{Pr2} when the code to cleanup validators after removing an admin was commented out.
Similarly, when we commented out a precondition that ensured that the number of validators should never fall below 2, we were able to create a sequence of transactions where \texttt{admin0} was able to vote itself out from the system, resulting in a livelock. 

The unknown bugs have been confirmed by the developer and have been fixed in the latest binary releases; the code on github will be updated in a future release. 
The complexity of several nested mappings, arrays, and inheritance required precise initialization of arrays and nested mappings to eliminate spurious aliasing between multiple mappings, or arrays at two different indices within a nested mapping. 
%script poa AdminValidatorSet 4 with /trackAllVars (w/o its running > 500s, w /trackAllVars also running > 600s, )
% running with 4 with the initial tracked variables, removed AdminSet invariants, 
Unlike the Workbench samples, we were only able to scale the bounded verification for the fixed contracts up to a transaction-depth of 4 (13 hours), with depth 3 taking 11 seconds.
The huge difference in time can be partially attributed to the difference in the number of procedures inlined by Corral (77 for depth 3 vs 831 for depth 4). 
%Program has no bugs
%Reached recursion bound of 4
%
%Boogie verification time: 48203.96 s
%Time spent reading-writing programs: 7.46 s
%
%Time spent checking a program (16): 48194.90 s
%Time spent checking a path (45): 24.29 s
%
%Number of procedures inlined: 831
%Number of variables tracked: 33
%Total Time: 48220.8863506 s
%Total User CPU time: 48191.78125 s
%
%script-demo poa AdminSet 8
For property \texttt{Pr4} that only involved the \texttt{AdminSet}, we were able to explore transaction depths 5, 6, 7 within 14, 50, 242 seconds respectively. %\Shuvendu{8} within \Shuvendu{300 seconds}. 



==> poa-eval.tex <==

%\subsubsection{Proof of Authority Governance Contracts}
\label{sec:poa-overview}

Separate from the application level Workbench offering, Azure Blockchain also offers ledger level services. One of them is Ethereum on Azure. The Ethereum blockchain comes with a choice of consensus protocols for a decentralized system: (i) the conventional {\it Proof of Work} (PoW) and the (ii) the {\it Proof of Authority} (PoA). 
%The consensus algorithm has to decide which node wins the privilege to append the latest block to the blockchain.

%The PoW is the widely used consensus algorithm for traditional public (permissionless) blockchain to guard against Sybil attacks in the presence of anonymous nodes, e.g., in the BitCoin network.
%A malicious party could easily create many nodes to be disproportionately powerful. 
%However, PoW consensus is computationally expensive as it relies on miners solving a difficult cryptographic puzzle, and therefore it limits the throughput (the number of transactions that can be mined per unit of time) of the blockchain network. 

While PoW is widely used, it suffers from malicious parties becoming disproportionately powerful by creating many nodes. Besides, PoW consensus is computationally expensive as it relies on miners solving a difficult cryptographic puzzle, and therefore it limits the throughput of the blockchain network. 

\begin{figure}[htbp]
\includegraphics[scale=0.4]{poa-governance.png}
\caption{POA Ethereum on Azure and its governance contracts.}
\label{fig:poa-ethereum-fig}
\end{figure}

The PoA is proposed as an alternative to PoW for permissioned consortium networks where the identities cannot be forged, as they are linked to off-chain identities. 
%It differs from a public blockchain in that the consortium is formed by running an election to accept new members, each having an identity. 
%The members share the resposibility/authority of validating transactions and appending them in the ledger. 
%It allows for a superior throughput in the case of consortium blockchain applications. 
%yet ensuring Byzantine fault tolerance. [Shuvendu, I am not sure if PoA ensures Byzantine fault tolerance. I remember Cody said that the validators just do round-robin. If not sure, we can remove "yet ensuring ..."]
%Enterprise customers and other systems such as Azure Blockchain Workbench can deploy a PoA network on Azure based on the Parity implementation of Ethereum.
The PoA network consists of a set of nodes running the PoA protocol and validating transactions. 
Every node is assigned a distinct Ethereum address, which is called the validator address. 
%The validator set is a contract managing a set of validator addresses (shown as "validators" for brevity). 
%Adding or removing a validator address will result in its corresponding node to be added into or removed from %the PoA network. 

%Parity Ethereum implementation exposes a {\it ValidatorSet} contract interface that is implemented by the Ethereum on Azure deployment. 
Governing a PoA network requires a set of contracts shown in Figure~\ref{fig:poa-ethereum-fig}. 
Validators belong to different organizations, such as companies A, B, and C in the figure. 
Each organization is represented by an admin contract. 
%Initially, the PoA network is created by one admin, who naturally becomes the only elected admin of the network. 
%Later, for another admin to become an elected admin, it needs to win a majority vote among existing elected admins. 
%An elected admin is allowed to bring in a number of validators. 
%The admins can also vote against each other. 
%If more than half of the existing elected admins vote against one of them, the admin will be evicted, and its validators are removed consequently.
Initially, the PoA network is created by one admin, and an admin could be elected or evicted based on the votes of other admins. An elected admin is allowed to bring in a number of validators.

The above protocol for admin voting and validator set management is implemented as a set of contracts that implement the Parity Ethereum's {\it ValidatorSet} contract interface, and available as part of Azure Blockchain content and samples~\cite{poa-cite,poa-github}.
It consists of five smart contracts (ValidatorSet, SimpleValidatorSet, AdminValidatorSet, Admin, AdminSet) totaling around 600 lines of Solidity code. 
%\begin{itemize}[leftmargin=*]
%\item {\bf ValidatorSet}: The interface that Parity client uses for determining authorities on the network
%\item {\bf SimpleValidatorSet}: A simple implementation of the ValidatorSet that handles adding validators . 
%\item {\bf AdminValidatorSet}: Inherits from SimpleValidatorSet, and introduces the concept of Admins for different organizations and voting.
%It allows an admin to control their validator set and vote for other admins.
%\item {\bf Admin}: A contract representing a Consortium member; it tracks votes for or against a given member.
%\item {\bf AdminSet}:  Contract used for performing constant time operations on a set of Admins. 
%\end{itemize}

The smart contracts use several features that make it a challenging benchmark for Solidity smart contract reasoning. 
We outline some of them here:
\begin{itemize}[leftmargin=*]
\item The contracts use  multiple levels of inheritance since the top-level contract \texttt{AdminValidatorSet} derives from the contract \texttt{SimpleValidatorSet} which in turn derives from \texttt{ValidatorSet} interface.
\item It uses sophisticated access control using Solidity modifiers to restrict which users and contracts can alter states of different contracts.
\item The contracts maintain deeply nested mappings and arrays to store the set of validators for different admins. 
\item The contracts use nested loops and procedures to iterate over the arrays and use arithmetic operations to reason about majority voting. 
\end{itemize} 




==> poa.tex <==

\subsubsection{Proof of Authority Governance Contracts}
\label{sec:poa-overview}

Separate from the application level Workbench offering, Azure Blockchain also offers ledger level services. One of them is Ethereum on Azure. The Ethereum blockchain comes with a choice of consensus protocols for a decentralized system: (i) the conventional {\it Proof of Work} (PoW) and the (ii) the {\it Proof of Authority} (PoA). 
The consensus algorithm has to decide which node wins the privilege to append the latest block to the blockchain.

The PoW is the widely used consensus algorithm for traditional public (permissionless) blockchain to guard against Sybil attacks in the presence of anonymous nodes, e.g., in the BitCoin network.
A malicious party could easily create many nodes to be disproportionately powerful. 
However, PoW consensus is computationally expensive as it relies on miners solving a difficult cryptographic puzzle, and therefore it limits the throughput (the number of transactions that can be mined per unit of time) of the blockchain network. 

\begin{figure}[htbp]
\includegraphics[scale=0.4]{poa-governance.png}
\caption{POA Ethereum on Azure and its governance contracts.}
\label{fig:poa-ethereum-fig}
\end{figure}

 

The PoA is proposed as an alternative to PoW for permissioned consortium networks where the identities cannot be forged, as they are linked to off-chain identities. 
It differs from a public blockchain in that the consortium is formed by running an election to accept new members, each having an identity. 
The members share the responsibility/authority of validating transactions and appending them in the ledger. 
It allows for a superior throughput in the case of consortium blockchain applications. 
%yet ensuring Byzantine fault tolerance. [Shuvendu, I am not sure if PoA ensures Byzantine fault tolerance. I remember Cody said that the validators just do round-robin. If not sure, we can remove "yet ensuring ..."]

Enterprise customers and other systems such as Azure Blockchain Workbench can deploy a PoA network on Azure based on the Parity implementation of Ethereum.
The network consists of a set of nodes running the PoA protocol and validating transactions. 
Every node is assigned a distinct Ethereum address, which is called the validator address. 
The validator set is a contract managing a set of validator addresses (shown as "validators" for brevity). 
Adding or removing a validator address will result in its corresponding node to be added into or removed from the PoA network. 

Parity Ethereum implementation exposes a {\it ValidatorSet} contract interface that is implemented by the Ethereum on Azure deployment. 
Governing a PoA network requires a set of contracts shown in Figure~\ref{fig:poa-ethereum-fig}. 
Validators belong to different organizations, such as companies A, B and C in the figure. 
Each organization is represented by an admin contract. 
Initially, the PoA network is created by one admin, who naturally becomes the only elected admin of the network. 
Later, for another admin to become an elected admin, it needs to win a majority vote among existing elected admins. 
An elected admin is allowed to bring in a number of validators. 
The admins can also vote against each other. 
If more than half of the existing elected admins vote against one of them, the admin will be evicted, and its validators are removed consequently.
The above protocol for admin voting and validator set management is implemented as a set of contracts that implement the Parity Ethereum's {\it ValidatorSet} contract interface, and available as part of Azure Blockchain content and samples~\cite{poa-cite,poa-github}.
It consists of the following smart contract implementations totaling around 600 lines of Solidity code. 
\begin{itemize}[leftmargin=*]
%\item {\bf ValidatorSet}: The interface that Parity client uses for determining authorities on the network
\item {\bf SimpleValidatorSet}: A simple implementation of the ValidatorSet that handles adding validators . 
\item {\bf AdminValidatorSet}: Inherits from SimpleValidatorSet, and introduces the concept of Admins for different organizations and voting.
It allows an admin to control their validator set and vote for other admins.
\item {\bf Admin}: A contract representing a Consortium member; it tracks votes for or against a given member.
\item {\bf AdminSet}:  Contract used for performing constant time operations on a set of Admins. 
\end{itemize}

The smart contracts use several features that make it a challenging benchmark for Solidity smart contract reasoning. 
We outline some of them here:
\begin{itemize}[leftmargin=*]
\item The contracts use  multiple levels of inheritance since the top-level contract \texttt{AdminValidatorSet} derives from the contract \texttt{SimpleValidatorSet} which in turn derives from \texttt{ValidatorSet} interface.
\item It uses sophisticated access control using Solidity modifiers to restrict which users and contracts can alter states of different contracts.
\item The contracts maintain deeply nested mappings and arrays to store the set of validators for different admins. 
\item The contracts make use of nested loops and procedures to iterate over the arrays, and make use of arithmetic operations to reason about majority voting. 
\end{itemize} 




==> soltoboogie.tex <==
\subsection{Encoding Solidity}
\label{sec:solidity}

In the next two sections, we describe the design of a formal verifier for Solidity smart contracts.
In this section, we first describe a translation of Solidity program to a program in the Boogie intermediate verification language~\cite{barnett-fmco05}.
Boogie has a small language with formalized semantics, such that verification tasks can be encoded into a formula in Satisfiability Modulo Theory (SMT), and can be discharged by SMT solvers such as Z3~\cite{z3}.
The ability to go from a Boogie program to a SMT formula allows us to leverage various bounded and unbounded verification techniques for Boogie.

\subsection{Boogie}
\label{sec:boogie}
We first describe a small subset of Boogie language that we use to formalize our translation from Solidity.

Boogie types are integers ($\bint$), references ($\bRef$) or arrays; arrays can be nested in that each index of an array can store an array. 
Booleans are syntactic sugar over integers. 
\newcommand{\bBaseTypes}{\mathit{BoogieElemTypes}}
\newcommand{\bBaseType}{\mathit{bbt}}
\newcommand{\bTypes}{\mathit{BoogieTypes}}
\newcommand{\bType}{\mathit{bt}}
\[
\begin{array}{lll}
\bBaseType \in \bBaseTypes & ::= & \ \bint  \ | \ \bRef \\
\bType \in \bTypes & ::= & \ \bBaseType \ | \ [\bBaseType]\bType
\end{array}
\]


\begin{figure}[!h]
\[
\begin{array}{lll}
\bexpr \in \Exprs & ::= & c \ | \  \varn{x}  \ | \  \bop{\bexpr,\ldots, \bexpr}  \ | \ \arrSel{\varn{x}}{e} \ | \ \forall i: \bBaseType :: \bexpr\\
\sstmt \in \Stmts &::=& \bskip \ | \ \bhavoc{\varn{x}} \ | \ \bassign{\varn{x}}{\bexpr} \ | \ \varn{x}[e]\ldots[e] := e \ | \  \\ 
                  &  & \bassume{\bexpr} \ | \ \bassert{\bexpr} \ | \  \\
                  &  & \bcall{\pproc}{\bexpr, \ldots, \bexpr}{\varnVector{x}} \ | \ \Seq{\sstmt}{\sstmt} \ | \\\
                  &  & \bifelse{\bexpr}{\sstmt}{\sstmt} \ | \ \bwhile{\bexpr}{\sstmt}
\end{array}
\]
\caption{Simple subset of Boogie language.}
\label{fig:boogie-lang}
\end{figure}


Figure~\ref{fig:boogie-lang} describes the expressions and statements in the language.
Expressions ($\Exprs$) consist of constants, variables, operations over expressions and array lookups, and quantified expressions.
Expressions can have one of the Boogie types described above, except $\forall$ expressions that have type Boolean. 
Standard statements ($\Stmts$) in Boogie consist of skip ($\bskip$), variable and array assignment, sequential composition, conditional statements, and loops.
The $\bhavoc{\varn{x}} \ $ statement assigns an arbitrary value of appropriate type to a variable $\varn{x}$.
A procedure call ($\bcall{\pproc}{\bexpr, \ldots, \bexpr}{\varnVector{x}}$) can return a vector of values that can be stored in local variables. 
The $\bassertn$ and $\bassumen$ statements behave as skip when the the Boolean valued argument evaluates to true in the state.
When the argument evaluates to false, then assert fails the execution and assume blocks the execution. 


%Types of expressions, can be \textit{Boolean}, \textit{integers}, or even \textit{maps}. 
%%We break up $\varn{x}[e_1][e_2]$ as $\bassign{\varn{y}}{\arrSel{\varn{x}}{e_1}}$ and $\arrSel{\varn{y}}{e_2}$. 
%[Note , we cannot desugar $\bassign{\varn{x}[e_1][e_2]}{e_3}$ as $\bassign{\varn{y}}{\arrSel{\varn{x}}{e_1}}$ and $\arrUpd{\varn{y}}{e_2}{e_3}$. ]

%The types of conditions in conditional statements restricted to Boolean valued expressions. 

A state $\sstate \in \States$ is a valuation of variables in scope.  
Evaluation of an expression $\bexpr \in \Exprs$, is denoted by $\eval{\bexpr}{\sstate}$, and defined inductively. 
We can define the standard operational (big-step) semantics $\step{\State{1}}{\sstmt}{\State{2}}$ that denotes that executing a statement $\sstmt \in \Stmts$ in a state $\State{1}$ can transition to a state $\State{2}$. 
We skip the details for the sake of brevity in this document.



\subsection{Solidity}

We now define a subset of Solidity language that is sufficiently expressive and yet concise enough to demonstrate the translation. 

\subsubsection{Types}

\newcommand{\typeMap}[1]{\beta(#1)}


\newcommand{\solTypes}{\mathit{SolTypes}}
\newcommand{\solType}{\mathit{st}}
\newcommand{\solBaseTypes}{\mathit{SolElemTypes}}
\newcommand{\solBaseType}{\mathit{et}}
\newcommand{\solContractTypes}{\mathit{ContractNames}}
\newcommand{\solContract}{\mathit{ct}}

We start with the set of Solidity types. 
Solidity types can be one of integer, string, address, a contract name, mappings or arrays over them. 
We unify a mapping type \texttt{mapping(t1 => t2)}  and an array type  \texttt{t2[t1]} in Solidity  as \texttt{t1} $\Rightarrow$ \texttt{t2}, where \texttt{t2} could be a nested array. 

\[
\begin{array}{lll}
\solContract \in \solContractTypes \\
\solBaseType \in \solBaseTypes & ::= & \ \intType \ | \ \stringType \ | \ \addrType \\
\solType \in \solTypes & ::= & \  \solBaseType \ | \ \solContract \ | \ \solBaseType \Rightarrow \solType
\end{array}
\]

We define a mapping $\mu: \solTypes \rightarrow \bTypes$ that translates a Solidity type to a type in Boogie as follows:
\[
\small{
\begin{array}{lll}
\mu({\solType}) & \doteq & \left\{
  \begin{array}{ll}
  \bint, & \solType \in \{\intType, \stringType\} \\
  \bRef, & \solType \in \{\addrType\} \cup \solContractTypes \\
  {[\mu(\solBaseType)]}\mu(\solType), & \solType \doteq \solBaseType \Rightarrow \solType \\
  \end{array}
  \right.
\end{array}
}
\]
As described later, we represent a Solidity string as an uninterpreted integer in Boogie.
Solidity by default treats a string as an uninterpreted value that can only be compared for equality. 

\subsubsection{Variables}


\newcommand{\this}{\texttt{this}}
\newcommand{\length}{\texttt{Length}}
\newcommand{\dtype}{\texttt{DType}}
\newcommand{\alloc}{\texttt{Alloc}}
\newcommand{\push}{\texttt{push}}

To model the semantics of an object-oriented language such as Solidity, each generated Boogie program consists of a set of variables in {\it global scope}:
\begin{itemize}
\item An array $\dtype: [\bRef]\solContractTypes$ that maps an address to a contract name corresponding to its dynamic type.
\item An array $\alloc: [\bRef]\bbool$ that maps an address to its allocation status.
\item An array $\length: [\bRef]\bint$ that maps the address (of an array) to the size of the array.
\item For each scalar state variable \varn{F} of type $t$ in a contract $C \in \solContractTypes$ in Solidity, we introduce a map $\texttt{F\_C}: [\bRef]\mu(t)$.
\item For an array or \texttt{mapping} state variable \varn{F}, we introduce a map $\texttt{F\_C}: [\bRef]\bRef$.
\item For any {\it array} type $t_1 \Rightarrow \ldots \Rightarrow t_k \Rightarrow t\in \solTypes$ (either as state variable or local variable) (where $t_i \in \solBaseTypes$ for $i \in [1,k]$), we add a set of maps:
\begin{itemize}
\item $\texttt{M\_bk\_b}: [\bRef][\mu(t_k)]\mu(t)$, and 
\item a set of at most $k-1$ distinct maps: 
$$\{\texttt{M\_bi\_Ref}:[\bRef][\mu(t_i)]\bRef \ | \ i \in [1, k-1]\}$$
\noindent Here $\texttt{bk}$ (respectively $\texttt{b}$) is the string representation of $\mu(t_k)$ (respectively $\mu(t)$); for example, if $\mu(t_k)$ is $\bint$, then $\texttt{bk}$ is ``int''.
\end{itemize}
\end{itemize}


\begin{figure*}[htbp]
\begin{minipage}[t]{0.45\textwidth}
\begin{lstlisting}[style=Sol]
// Solidity code with nested mappings
// inheritance, constructor and require
pragma solidity ^0.4.24;
contract A {
    mapping (int => int[]) n;
    constructor() {
       n[0].push(22);
    }
    function F() returns (bool) {
        return false;
    }
}
contract B is A {
    mapping (int => int) m;
    constructor()  {
	require (n[0].length == 1);
        m[0] = 11;
        m[1] = 21; 
        //m[0] does not alias m[1]
        assert (m[0] == 11);
        //n[0][0] does not alias m[*]
        assert (n[0][0] == 22); 
    }
    function F() returns (bool) {
        return true;
    }
}
contract C {
   A a;
   constructor() {
      a = new B();      
      assert(a.F());
   }
}
\end{lstlisting}
\caption{Solidity source code}
\label{fig:solidity-source-code}
\begin{lstlisting}[style=Boogie, basicstyle=\ttfamily \scriptsize]
// global declarations
type Ref;
type ContractName;
var DType: [Ref]ContractName;
var Alloc: [Ref]bool;
var M_int_int: [Ref][int]int;
var M_int_Ref: [Ref][int]Ref;
var Length: [Ref]int;
procedure Fresh(): (newRef: Ref){
  havoc newRef; assume (!Alloc[newRef]);
  Alloc[newRef] := true;
}
procedure HavocAllocMany() {
   var oldAlloc: [Ref]bool; 
   oldAlloc := Alloc; havoc Alloc;
   assume ($\forall$ i:Ref :: oldAlloc[i] ==> Alloc[i]);
}
\end{lstlisting}
\caption{Boogie prelude}
\label{fig:boogie-prelude}
\end{minipage}
\begin{minipage}[t]{0.45\textwidth}
\begin{lstlisting}[style=Boogie,basicstyle=\ttfamily \scriptsize]
// Boogie code 
const unique A, B, C: ContractName;

var n_A, m_B, a_C: [Ref]Ref;

// A's constructor
proc A_Ctor(this: Ref, msg_sender: Ref) {
   // start of initialization
   // Make array/mapping vars distinct for n
   call tmp := Fresh(); $\label{line:init-start}$

   // nested array initialization
   assume ($\forall$  i:int :: (Length[M_int_Ref[tmp][i]] == 0));
   assume ($\forall$  i:int :: !(Alloc[M_int_Ref[tmp][i]])); $\label{line:init-start2}$
   call HavocAllocMany(); $\label{line:init-havocmany}$
   assume ($\forall$  i:int :: Alloc[M_int_Ref[tmp][i]]); $\label{line:init-start3}$
   assume ($\forall$  i, j:int :: (i == j ||               
           M_int_Ref[tmp][i] != M_int_Ref[tmp][j])); $\label{line:init-end}$
   assume ($\forall$  i:int, j:int :: 
           M_int_int[M_int_Ref[tmp][i]][j] == 0);  $\label{line:init-end2}$
   n_A[this] := tmp;
   // end of initialization

   var l := Length[M_int_Ref[n_A[this]][0]];
   M_int_int[M_int_Ref[n_A[this]][0]][l] := 22;
   Length[M_int_Ref[n_A[this]][0]] := l + 1;
}
proc F_A(this:Ref, msg_sender: Ref) returns (r:bool) {
   r := false;
}
// B's constructor
proc B_Ctor(this: Ref, msg_sender: Ref) {
   call A_Ctor(this, msg_sender);

  // start of initialization
  // Make array/mapping vars distinct for m
  call tmp := Fresh();
  // Initialize Integer mapping m
  assume (forall  i:int :: M_int_int[tmp][i] == 0);
  m_B[this] := tmp;
  // end of initialization
  
  assume (Length[M_int_Ref[n_A[this]][0]] == 1);
  M_int_int[m_B[this]][0] := 11;
  M_int_int[m_B[this]][1] := 21;
  assert (M_int_int[m_B[this]][0] == 11);
  assert (M_int_int[M_int_Ref[n_A[this]][0]][0] == 22);
}
proc F_B(this:Ref, msg_sender: Ref) returns (r:bool) {
   r := true;
}
// C's constructor
proc C_Ctor(this: Ref, msg_sender: Ref) {
   call x := Fresh();
   assume (DType[x] == B);
   call B_Ctor(x, this);
   a_C[this] := x;
   if (DType[a_C[this]] == B) { /* dyn dispatch */
      call y := F_B(a_C[this], this); /* msg.sender update */
   } else if (DType[a_C[this]]) == A) {
      call y := F_A(a_C[this], this);
   }
   assert (y);
}

\end{lstlisting}
\caption{Translated Boogie code.}
\label{fig:boogie-translation}
\end{minipage}
\caption{Example Solidity code and translated Boogie code that includes the program-independent prelude and program-specific translation.}
\label{fig:Solidity-To-Boogie}
\end{figure*}


%[Provide the translation as a set of inference rules]
Consider the example contracts in Figure~\ref{fig:Solidity-To-Boogie} to illustrate the modeling. 
\begin{itemize}[leftmargin=*]
\item First, for the state variable \texttt{a} in contract \texttt{C} of scalar type $\texttt{A} \in \solContractTypes$, we introduce a map \texttt{a\_C} of type $[\bRef]\bRef$; an access to \texttt{a} inside a contract instance is treated as $\arrSel{\texttt{a\_C}}{\this}$.
Here $\this$ is a parameter to the enclosing method to refer to the address of the current object or contract instance (corresponds to Solidity $\this$). 
\item Second, since there is an array type $\bint \Rightarrow \bint \Rightarrow \bint \in \solTypes$ in the program as the type of \texttt{n} in contract \texttt{A}, we introduce the maps \texttt{M\_int\_Ref: [Ref][int]Ref} and \texttt{M\_int\_int:[Ref][int]int}. 
\item An array access in Solidity such as \texttt{n}[0][0] is translate as 
$$\texttt{M\_int\_int[M\_int\_Ref[n\_A[this]][0]][0]}$$
where \texttt{n\_A[this]} looks up the value of \texttt{n} for this instance, \texttt{M\_int\_Ref[n\_A[this]][0]} looks up the map at index 0, which is finally used to index into the \texttt{M\_int\_Ref} map again at index 0 to obtain the scalar value. 
We define the formal translation of expressions later in this section. 
\end{itemize}

In addition to the set of globals, the set of variables in {\it local scope} consists of 
\begin{itemize}
\item A formal parameter $\varn{x}$ of type $\mu(t)$ for each solidity parameter $\varn{x}$ of type $t$.
\item A formal parameter \texttt{msg\_sender} of type $\bRef$, and a formal parameter \texttt{this} of type $\bRef$. These variable models the implicit Solidity parameters $\texttt{msg.sender}$ and $\this$ respectively.
\item A local variable $\varn{x}$ of type $\mu(t)$ for each Solidity local variable $\varn{x}$ of type $t$.
\end{itemize} 


\subsubsection{Expressions}

\begin{figure}[!h]
\[
\begin{array}{lll}
\solExpr{} \in \solExprs & ::= & c \ | \  \varn{x}  \ | \  \bop{\solExpr{},\ldots, \solExpr{}}  \ | \ \arrSel{\varn{x}}{\solExpr{}} \ | \ \varn{x.length}\\
\solStmt{} \in \solStmts &::=&  \bassign{\varn{x}}{\solExpr{}} \ | \ \varn{x}[\solExpr{}] := \varn{y} \ | \ \Seq{\solStmt{}}{\solStmt{}} \ | \ \\ 
                  &  & \solRequire(\solExpr{}) \ | \ \solAssert(\solExpr{}) \ | \  \\
                  &  & \solIfelse{\solExpr{}}{\solStmt{}}{\solStmt{}} \ | \ \\
                  &  & \solWhile{\solExpr{}}{\solStmt{}} \ | \ \varn{x}.\push(\solExpr{}) \ | \ \\
                  &  & \varn{x} = \texttt{Foo}(\vec{\solExpr{}}) \ | \ \varn{x} = \varn{y}.\texttt{Foo}(\vec{\solExpr{}}) \ | \ \\ 
                  &  & \varn{x}  =  \texttt{new} \ C(\vec{\solExpr{}}) \ | \ \varn{x}  =  \texttt{new}  \ t[](\solExpr{}) \ | \ \\
                  &  & \varn{x}  =  \texttt{new} \ (t_1 \Rightarrow t)()\ | \  \varn{x}  =  \texttt{new} \ (t_1 \Rightarrow (t_2 \Rightarrow t))()\\
\end{array}
\]
\caption{Simple subset of Solidity language.}
\label{fig:solidity-lang}
\end{figure}

\newcommand{\transExprn}{\Gamma}
\newcommand{\transExpr}[1]{\transExprn(#1)}
\newcommand{\transStmtn}{\Delta}
\newcommand{\transStmt}[1]{\transStmtn(#1)}
\newcommand{\strToInt}[1]{\textit{StrToInt}(#1)}
\newcommand{\solTypeOf}[1]{\textit{SolTypeOf}(#1)}

\begin{figure*}
\small
\[
\begin{array}{lll}
\transExpr{c} & \doteq & \left\{
  \begin{array}{ll}
  c, & \textrm{if } c \textrm{ is an integer, address constant literal}\\
  \strToInt{c}, & \textrm{if } c \textrm{ is a string constant literal}\\
  \end{array}
  \right. \\
\transExpr{\varn{x}} & \doteq & \left\{
  \begin{array}{ll}
  \varn{x}, & \textrm{if \varn{x} is a local or parameter} \\
  \varn{msg\_sender}, & \textrm{if \varn{x} is \varn{msg.sender}} \\
  \texttt{x\_C}[\this], & \textrm{if \varn{x} is a state variable in contract } $C$
  \end{array}
  \right. \\
\transExpr{\bop{\solExpr{1},\ldots, \solExpr{k}}} & \doteq & \bop{\transExpr{\solExpr{1}},\ldots, \transExpr{\solExpr{k}}} \\
\transExpr{\arrSel{\varn{x}}{\solExpr{}}} & \doteq & \left\{
  \begin{array}{ll}
  \texttt{M\_t\_Ref}[\transExpr{\varn{x}}][\transExpr{\solExpr{}}], &\textrm{if $\mu(\solTypeOf{\solExpr{}})$ is \texttt{t} and $\varn{x}[\solExpr{}]$ is array type} \\
  \texttt{M\_t\_t2}[\transExpr{\varn{x}}][\transExpr{\solExpr{}}], &\textrm{if $\mu(\solTypeOf{\solExpr{}})$ is \texttt{t} and $\mu(\solTypeOf{\varn{x}[\solExpr{}]})$ is \texttt{t2}} 
  \end{array}
  \right. \\
\transExpr{\texttt{x.length}} & \doteq & \length[\transExpr{\varn{x}}]\\
\transExpr{\vec{\solExpr{}}} & \doteq & \transExpr{\solExpr{0}}, \ldots , \transExpr{\solExpr{k-1}}, \ \textrm {where $k$ = |$\vec{e}$|}
\end{array}
\]
\caption{Translation of Solidity expressions to Boogie.}
\label{fig:translate-sol-expr}
\end{figure*}


Figure~\ref{fig:solidity-lang} describes the set of Solidity expressions ($\solExprs$).
Most expressions are standard; the expression $\texttt{x.length}$ refers to the length of a static or dynamically allocated array $\varn{x}$. 
Figure~\ref{fig:translate-sol-expr} describes translation of a Solidity expression (denoted by the function $\transExpr{}: \solExprs \rightarrow \Exprs$) to an expression in Boogie. 
We highlight the non-trivial cases here.
For a string literal, we use an uninterpreted function $\strToInt$ to map it to an integer; one can think of this as a hash of the string. 
For a state variable $\varn{x}$ in contract $C$, the translation $\transExpr{\varn{x}}$ indexes into $\varn{x}\_C$ with the $\this$ parameter. 
The translation of array access $\arrSel{\varn{x}}{\solExpr{}}$ indexes into a global array after recursively translating $\varn{x}$ and $\solExpr{}$. 
The choice of array depends on the Solidity type of $\varn{x}[\solExpr{}]$.
If the Solidity type is an array then the resulting expression has type $\bRef$ in Boogie to represent the address of such an array; we index into the array $\texttt{M\_t\_Ref}$.
Otherwise, we index into the array $\texttt{M\_t\_t2}$ where $\texttt{t2}$ is the translated type of $\varn{x}[\solExpr{}]$. 

\subsubsection{Statements}
\begin{figure*}
\small
\[
\begin{array}{lll}
\transStmt{\solRequire(\solExpr{})} & \doteq & \bassume(\transExpr{\solExpr{}})\\
\transStmt{\solAssert(\solExpr{})} & \doteq & \bassert(\transExpr{\solExpr{}})\\
\transStmt{\varn{x} \ = \ {\solExpr{}}} & \doteq & \left\{
  \begin{array}{ll}
  \bassign{\transExpr{\varn{x}}}{\transExpr{\solExpr{}}}, & \textrm{if \varn{x} is a scalar variable, or the assignment is by reference} \\
%  \bfont{let} \ \textit{ArrayCopy}(\varn{a}, \varn{b}, \varn{len}) \ = & \textrm{Otherwise, perform an array copy} \\
%  \ \texttt{int \varn{i} := 0}; & \\
%  \ \bwhilen(\varn{i} < \varn{len}) \ \{ \ \varn{a}[\varn{i}] := \varn{b}[\varn{i}]; \ \varn{i} := \varn{i} + 1; \ \} & \\
%  \bfont{in} & \\
%  \ \ \textit{ArrayCopy}(\transExpr{\varn{x}}, \transExpr{e}, \length({\transExpr{\varn{x}}})) & \\
%  \bfont{end} & 
  \bot, & \textrm{throw an exception for any deep copy}
\end{array}
\right. \\
%\transStmt{\varn{x}[\solExpr{}] \ = \ \varn{y}} & \doteq & \left\{
%  \begin{array}{ll}
%  \texttt{M\_t\_Ref}[\transExpr{x}][\transExpr{\solExpr{}}] := \transExpr{\varn{y}}, &\textrm{if $\mu(\solTypeOf{\solExpr{}})$ is \texttt{t} and \varn{x}[$\solExpr{}$] is array type} \\
%  \texttt{M\_t\_t2}[\transExpr{x}][\transExpr{\solExpr{}}] := \transExpr{\varn{y}}, &\textrm{if $\mu(\solTypeOf{\solExpr{}})$ is \texttt{t} and $\mu(\solTypeOf{\varn{x}[\solExpr{}]})$ is \texttt{t2}} 
%  \end{array}
%  \right. \\
%
\transStmt{\varn{x}[\solExpr{}] \ = \ \varn{y}} & \doteq & \transExpr{\varn{x}[\solExpr{}]} := \transExpr{\varn{y}}\\
%
\transStmt{\Seq{\solStmt{1}}{\solStmt{2}}} & \doteq & \Seq{\transStmt{\solStmt{1}}}{\transStmt{\solStmt{2}}} \\
%
\transStmt{\solIfelse{e}{s_1}{s_2}} & \doteq & \bifelse{\transExpr{e}}{\transStmt{s_1}}{\transStmt{s_2}}\\
%
\transStmt{\solWhile{e}{s}} & \doteq & \bwhile{\transExpr{e}}{\transStmt{s}}\\
%
\transStmt{\varn{x} \ = \ \texttt{Foo}(\vec{e})} & \doteq & \{ \ \bcall{\texttt{Foo}}{\this, \transExpr{\vec{e}}, \texttt{msg\_sender}}{\varn{tmp}} ; \ \transExpr{\varn{x}} := \varn{tmp}; \ \}, \ \ \ \textrm{// internal function call and static dispatch}\\
%
%\transStmt{\varn{x} \ = \ \varn{y}.\texttt{Foo}(\vec{e})} & \doteq & \bcall{\texttt{Foo}}{\transExpr{\varn{y}}, \transExpr{\vec{e}}, \this}{\transExpr{\varn{x}}}, \ \ \ \textrm{// external call, \varn{x} is a scalar type, \varn{y} is a contract instance or ``\this''} \\
%
\transStmt{\varn{x} \ = \ \varn{y}.\texttt{Foo}(\vec{e})} & \doteq & \textrm{// external call, dynamic dispatch} \\
&& \{ \\
&& \ \ \ \bfont{if} \ (\dtype[{\transExpr{\varn{y}}}] == A) \ \{ \bcall{\texttt{Foo}_A}{\transExpr{\varn{y}}, \transExpr{\vec{e}}, \this}{\varn{tmp}}; \ \transExpr{\varn{x}} := \varn{tmp}; \}\\
&& \ \ \ \bfont{else} \ \bfont{if} \ (\dtype[{\transExpr{\varn{y}}}] == B) \ \{ \bcall{\texttt{Foo}_B}{\transExpr{\varn{y}}, \transExpr{\vec{e}}, \this}{\varn{tmp}}; \ \transExpr{\varn{x}} := \varn{tmp}; \}\\
&& \ \ \ \ldots \\
&& \ \ \ \bfont{else} \ \{ \ \bassume{\bfalse}; \ \} \\
&& \} \\
%
\transStmt{\varn{x}.\push(\solExpr{})} & \doteq & \transStmt{\varn{x}[\varn{x.length} \texttt{++}] = \solExpr{}; } \ \textrm{//pushing a new array element} \\
%
\transStmt{\varn{x} \ = \ \texttt{new} \ t[](\solExpr{})} & \doteq &  \ \textrm{//allocating a new dynamic array of type $t \in \solBaseTypes$} \\
&& \{\bcall{\texttt{Fresh}}{}{\varn{tmp}}; \length[\varn{tmp}] := \transExpr{\solExpr{}}; 
   \bassume{(\forall i: \bint :: \texttt{M\_Int\_t}[\varn{tmp}][i] == 0)}; \transExpr{\varn{x}} := \varn{tmp}; \}\\
%
\transStmt{\varn{x} \ = \ \texttt{new} \ (t_1 \Rightarrow t)()} & \doteq &  \ \textrm{//initializing a mapping $t_1 \Rightarrow t$ s.t. \texttt{t1} is $\mu(t_1)$} \\
&& \{\bcall{\texttt{Fresh}}{}{\varn{tmp}}; \bassume{(\forall i: \mu(t_1) :: \texttt{M\_t1\_t}[\varn{tmp}][i] == 0)}; \transExpr{\varn{x}} := \varn{tmp}; \}\\
%
\transStmt{\varn{x} \ = \ \texttt{new} \ (t_1 \Rightarrow (t_2 \Rightarrow t))()} & \doteq &  \ \textrm{//initializing a mapping $t_1 \Rightarrow (t_2 \Rightarrow t)$ s.t. \texttt{ti} is $\mu(t_i)$ and \texttt{t} is $\mu(t)$} \\
&& \{ \\
&& \ \ \ \bcall{\texttt{Fresh}}{}{\varn{tmp}}; \\
&& \ \ \ \bassume{(\forall i: \mu(t_1) ::  \texttt{Length(M\_t1\_Ref)}[\varn{tmp}][i]) == 0}; \\
&& \ \ \ \bassume{(\forall i: \mu(t_1) :: \neg \texttt{Alloc}(\texttt{M\_t1\_Ref}[\varn{tmp}][i]}; \\
&& \ \ \ \bcalln \ \texttt{HavocAllocMany}(); \\
&& \ \ \ \bassume{(\forall i: \mu(t_1) ::  \texttt{Alloc}(\texttt{M\_t1\_Ref}[\varn{tmp}][i]}; \\
&& \ \ \ \bassume{(\forall i, j: \mu(t_1) :: (i == j  \vee \texttt{M\_t1\_Ref}[\varn{tmp}][i] \neq \texttt{M\_t1\_Ref}[\varn{tmp}][j])}; \\
&& \ \ \ \bassume{(\forall i: \mu(t_1), j:\mu(t_2) :: \texttt{M\_t2\_t}[\texttt{M\_t1\_Ref}[\varn{tmp}][i]][j] == 0)}; \\
&& \ \ \ \transExpr{\varn{x}} := \varn{tmp}; \\
&& \}\\
%
\transStmt{\varn{x} \ = \ \texttt{new} \ C(\vec{\solExpr{}})} & \doteq &  \textrm{//$C \in \solContractTypes$} \\
&&  \{ \bcall{\texttt{Fresh}}{}{\varn{tmp}}; \
   \bassume{\dtype(\varn{tmp}) == C}; \
   \bcalln \ \texttt{C\_Ctor}(\varn{tmp}, \transExpr{\vec{\solExpr{}}}, \this); \
   \transExpr{\varn{x}} := \varn{tmp}; \}\\
%
\end{array}
\]
\caption{Translation of Solidity statements to Boogie. We do not translate statements that involve a deep copy.}
\label{fig:translate-sol-stmt}
\end{figure*}

Figure~\ref{fig:solidity-lang} also describes the set of statements in Solidity that we translate to Boogie.
The $\solRequire(\solExpr{})$  aborts execution when executed in a state when $\solExpr{}$ is false, and can be used for adding preconditions to functions.
In contrast, $\solAssert(\solExpr{})$ is used to terminate execution when an internal invariant $\solExpr{}$ does not hold. 
We distinguish between two types of procedure calls (a) {\it internal} call $\varn{x} \ = \ \texttt{Foo}(\vec{e})$ which invokes a method $\texttt{Foo}$ within the same contract, and (b) {\it external} call  $\varn{x} \ = \ \varn{y}.\texttt{Foo}(\vec{e})$ that invokes a method on a contract instance pointed to by $\varn{y}$ (which may include $\this$).
For an array variable $\varn{x}$, $\varn{x}.\push(\solExpr{})$ adds an element with value $\solExpr{}$ to the end of the array and increments the $\varn{x}.\texttt{length}$. 
We support two types of dynamic allocation (i) creation of a new contract instance of type $C$ through $\varn{x}  =  \texttt{new} \ C(\vec{\solExpr{}})$ and (ii) allocating an array of $\solBaseTypes$ type $t$ of size $\solExpr{}$ through $\varn{x}  =  \texttt{new}  \ t[](\solExpr{})$. 
Finally, we support the implicit allocation of a nested mapping of type $t_1 \Rightarrow \ldots (t_k \Rightarrow t)$ using  $\varn{x}  =  \texttt{new} \ (t_1 \Rightarrow t)()$ and $\varn{x}  =  \texttt{new} \ (t_1 \Rightarrow (t_2 \Rightarrow t))()$ to show the first two levels for $k \in [1, 2]$. 


\begin{figure}[htbp]
\centering
\includegraphics[scale=0.7]{arraysemantics.png}
\vspace{-0.1in}
\caption{Semantics of Solidity array assignment LHS = RHS.}
\label{fig:sol-arr-semantics}
\end{figure}

\paragraph{\bf Assignments.} Figure~\ref{fig:translate-sol-stmt} provides the translation of Solidity statements to Boogie statements using the function $\transStmtn$.
We translate $\solRequire(\solExpr{})$ (respectively $\solAssert(\solExpr{})$) using $\bassumen$ (respectively, $\bassertn$), given that these statements terminate execution when the argument is false and we do not allow exceptions to be caught in our subset of Solidity. 
An assignment $\varn{x} = \solExpr{}$ in Solidity can either be a simple top-level assignment (of a value or address) or a deep-copy (in the case of certain arrays).
Figure~\ref{fig:sol-arr-semantics} shows the cases where an array assignment in Solidity is treated as assigning the reference (\texttt{Ref}) or performing a deep-copy (\texttt{Deep})~\cite{solidity-assignment-cite}.
Our translator currently does not handle programs that contain deep copy; this is denoted by the $\bot$ when we encounter the need for a deep copy. 
Translation of an array assignment $\transStmt{\varn{x}[\solExpr{}] \ = \ \varn{y}}$ (that does not correspond to a deep-copy) uses $\transExpr{\varn{x}[\solExpr{}]}$ to determine the array to be updated. 

\paragraph{\bf Functions.} A function in Boogie has two additional input parameters that correspond to the implicit parameters in a Solidity function.
We add a first formal parameter with the name $\texttt{this}$ that holds the value the receiver object, and the last formal parameter with the name $\texttt{msg\_sender}$ that holds the user or contract address ($\texttt{msg.sender}$ in Solidity) that invokes the function.
The translation of internal function calls is more or less straightforward; note that the $\texttt{msg\_sender}$ is unchanged for an internal call.
An external call first needs to perform a case-split based on the dynamic type of the receiver object to handle dynamic dispatch due to inheritance; we assume a closed program where all the types are known at compile time. 
Recall that the dynamic type of an object is stored in the $\dtype$ array. 
Once the dynamic type $\dtype[\transExpr{\varn{y}}]$ is determined (say $B$), the call is dispatched to the copy of \texttt{Foo} (say, $\texttt{Foo}_B$) that is in scope for the dynamic type. 
For a given type, the \texttt{Foo} in scope may be defined in one of the base contracts. 
Since Solidity supports multiple inheritance, we traverse the list of {\it linearized} base contracts (as provided by the compiler) to find the first function with matching signature as \texttt{Foo} starting from the most derived contract.  
Note that value of the $\sender$ is changed to $\this$ to reflect that the sender is a contract. 
The $\push$ operation is desugared in terms of simpler statements. 

\paragraph{\bf Dynamic Allocation.} Dynamic arrays and contract allocations are handled using a helper Boogie procedure $\texttt{Fresh}$ (defined in ``Boogie Prelude'' Fig~\ref{fig:Solidity-To-Boogie}) that assigns a fresh non-allocated address.
The Boogie procedure $\texttt{Fresh}$ uses the global variable $\alloc$ to return a previously unallocated fresh reference $\varn{newRef}$.
For dynamic array allocation of a an array of type $t$ ($\texttt{new} \ t[](\solExpr{})$), we initialize the $\length$ of the array as well as the contents. 

We treat the initialization of mappings as implicit dynamic allocations as well.
We discuss the implicit allocation of a nested mapping of type $\varn{x}  =  \texttt{new} \ (t_1 \Rightarrow \ldots (t_k \Rightarrow t))()$ for the first two levels for $k \in [1, 2]$. 
The modeling of $\texttt{new} \ (t_1 \Rightarrow t)$ is identical to $\texttt{new} \ t[](\solExpr{})$, except $\length$ is not defined for a mapping. 

For the allocation $\texttt{new} \ (t_1 \Rightarrow (t_2 \Rightarrow t))()$, we need to ensure several disjointness conditions: 
(i) the address of freshly allocated $\varn{tmp}$ does not alias any other previously allocated address, and 
(ii) for any index $i$, the address of the nested arrays $\texttt{M\_t1\_Ref}[\varn{tmp}][i]$ do not alias (a) any other previsouly allocated address, and (b) the address of nested arrays $\texttt{M\_t1\_Ref}[\varn{tmp}][i]$ and $\texttt{M\_t1\_Ref}[\varn{tmp}][j]$ do not alias when distinct $i$ and $j$.
The challenge here is to ensure non-aliasing of an unbounded set of addresses.
This is achieved by a call to $\texttt{HavocAllocMany}$ helper procedure (part of the Boogie prelude in sub Figure~\ref{fig:boogie-prelude}); this procedure freshly allocates an unbounded set of addresses while retaining the old allocated addresses. 
The pair of assume statements preceding and following the call to $\texttt{HavocAllocMany}$ ensure that the addresses of nested arrays do not alias with any previously allocated address.
The next assume states that the nested arrays for any pair of distinct indices $i$ and $j$ are distinct. 
The final assume zero initializes the contents of the nested arrays. 
%The procedure call in line~\ref{line:init-havocmany} along with the three assume statements in lines~\ref{line:init-start2},~\ref{line:init-start3} and~\ref{line:init-end} ensure the desired disjointness. 

We informally sketch the generalization to arbitrarily deep nested mappings $\texttt{new} \ (t_1 \Rightarrow \ldots (t_k \Rightarrow t))()$ next.
For each level $t_i \in [t_1,\ldots,t_k]$, we invoke $\texttt{HavocAllocMany}$ and install similar assumptions for ensuring non-aliasing of nested addresses at level $i$ with any previously allocated addresses. 
Finally, for the last level $k$, we will zero initialize the contents. 


Contract allocation of type $C$ invokes $\texttt{Fresh}$ to allocate a fresh address, sets the dynamic type of the address and then calls the constructor $\texttt{C\_Ctor}$ with appropriate arguments and returns the fresh address.
A call to a constructor function $\texttt{C\_Ctor}$ has several steps: (i) executes the constructors of the base classes in the linearized order of inheritance, (ii) allocates and initializes the static state variables including arrays and mappings, and (iii) executes the statements in $\texttt{C\_Ctor}$. 

\begin{example}
%\paragraph{\bf Disjointness and Initialization.} 
We briefly go over the set of initializations that we perform in the constructor using an example; by default, values are unconstrained retaining soundness.
Figure~\ref{fig:Solidity-To-Boogie} illustrates a simple Solidity program (sub Figure~\ref{fig:solidity-source-code}), and the translated Boogie program (sub Figures~\ref{fig:boogie-prelude} and ~\ref{fig:boogie-translation}). 
The example is inspired by the PoA governance contracts (Section~\ref{sec:poa-overview}) that contain several nested mappings and array state and local variables.
Ensuring initialization and non-aliasing of nested arrays and mappings at contract allocation is crucial for establishing any non-trivial property. 
The assertions present in the constructor of contract $B$ model several such example non-aliasing properties. 
For this example, we only describe the initialization within the constructors; the translation of the remaining statements follow a straightforward application of $\transStmtn$ to each Solidity statement. 
Consider the constructor $\texttt{A\_Ctor}$ for contract $A$.
$A$ has a nested mapping $\varn{n}$ from integers to an array of integers; we treat it as $\intType \Rightarrow (\intType \Rightarrow \intType)$ mapping.
Lines~\ref{line:init-start} to ~\ref{line:init-end2} in Figure~\ref{fig:boogie-translation} perform initialization related to $\varn{n}$.
\end{example}

\subsubsection{Features in progress}

We currently handle a subset of the  Solidity language. 
Most of the unhandled features are orthogonal to the current translation, and thus can be added modularly.
We discuss some of these missing features in the current translation.
First, we are working on designing a sound semantics for the deep-copy array assignments; we currently require simplifying the source code to turn such assignments into a assignment of references. 
Second, we do not support low-level call statements using $\texttt{call}$ that looks up a function using a hash of the signature; such calls are discouraged in favor of high-level procedure calls that we support~\cite{discourage-call-solidity}.
Third, we do not support \texttt{balance} related logic for \texttt{payable} contracts for exchanging ether, including \texttt{send} and \texttt{transfer} operations; interestingly, many enterprise workflow related contracts do not use payable contracts and instead use an implementation of some standard tokens (e.g. \texttt{ERC20}). 
Finally, we also currently do not support modifiers, libraries, structs and inlined assembly instructions. 
Recall that our semantic conformance checking in Section~\ref{sec:solidity-instrumentation} used modifiers to add the runtime checks. 
Our current implementation uses a slightly more involved variant using a derived class to add similar checks without the need for modifiers. 
We plan to add modifiers to our translation soon as it is fairly common way to enforce preconditions including access control.  
We currently do not distinguish the different variants of integers such as unsigned integers or integers of fixed width, and model them all as unbounded integers. 

%\Shuvendu{Omit modifiers and instrumentation, libraries, structs, payable related attributes, send/transfer, fallback, low-level calls (not advised), ...}

%\begin{itemize}
%\item type mapping (int, bool, refs)
%\item expressions
%\item control flow (standard)
%\item this, msg.sender
%\item contract allocation 
%\item calls (internal, external, high-level, ..)
%\item exceptions, require, assert
%\item inheritance, virtual dispatch, constructor
%\item arrays and mapping
%\item dynamic arrays, push, length, ..
%\item array initialization 
%\item array assignments and copy semantics (different combinations)
%\end{itemize}



==> workbench.tex <==
\newcommand{\Appl}{\it{App}}
\newcommand{\Roles}[1]{\mathcal{R}_{#1}}
\newcommand{\role}[1]{\mathit{r}_{#1}}
\newcommand{\Workflows}[1]{\mathcal{W}_{#1}}
\newcommand{\workflow}[1]{\mathit{w}_{#1}}
\newcommand{\WfStates}[1]{\mathcal{S}_{#1}}
\newcommand{\WfState}[1]{\mathit{s}_{#1}}
\newcommand{\WfStateVar}{\mathit{State}}
\newcommand{\WfProperties}[1]{\mathcal{P}_{#1}}
\newcommand{\WfInstanceProperties}[1]{\mathcal{Q}_{#1}}
\newcommand{\WfInstanceProperty}[1]{\mathit{q}_{#1}}
\newcommand{\WfProperty}[1]{\mathit{p}_{#1}}
\newcommand{\WfInitState}[1]{\WfState{#1}^0}
\newcommand{\WfFunctions}[1]{\mathcal{F}_{#1}}
\newcommand{\WfFunction}[1]{\mathit{f}_{#1}}
\newcommand{\Types}[1]{\mathcal{T}_{#1}}
\newcommand{\type}[1]{\mathit{t}_{#1}}
\newcommand{\param}[1]{\mathit{x}_{#1}}
\newcommand{\WfTransitions}[1]{\mathcal{\gamma}_{#1}}
\newcommand{\Identifier}[1]{\mathit{id}_{#1}}
\newcommand{\AccessControl}[1]{\mathcal{AC}_{#1}}
\newcommand{\accessSet}[2]{\mathit{ac}_{#2}^{#1}}
\newcommand{\WfRoleRegistry}{\mathtt{RoleRegistry}}
\newcommand{\sender}{\mathit{sender}}

\newcommand{\translateAC}[1]{\pi(#1)}
\newcommand{\translatePostStates}[1]{\alpha(#1)}


\newcommand{\intType}{\mathit{integer}}
\newcommand{\stringType}{\mathit{string}}
\newcommand{\addrType}{\mathit{address}}


\subsection{Workbench Application Policy}
\label{sec:workbench-interface}

The Workbench application policy (\workbenchInterface) is described in a JSON file. 
The \workbenchInterface{} for an application allows the user to describe (i) the {\it data members} and {\it actions} of an applications, (ii) a high-level {\it state-machine} view of the application, and (iii) role-based {\it access control} for {\it state transitions}  of the application.
The role-based access control provides security for deploying smart contracts in an open and adversarial setting; 
the high-level state machine naturally captures the essence of a {\it workflow} that progresses between a set of states based on some actions from the user.

We assume that each function (or action) is associated with a $\sender{}$, which is the address of a user or another workflow that invokes the function. 
In Solidity, this is denoted by {\texttt msg.sender} parameter within a function. 
The invocation of a function in a given state can be restricted to users that belong to certain roles --- we refer to this as the {\it access control}. 

Formally, a {\it Workbench Application Policy} $\Appl(\Roles{}, \Workflows{}, \Types{})$ consists of the following:
\begin{itemize}[leftmargin=*]
\item $\Roles{}$: a set of {\it global roles} used for access control.
\item $\Types{}$: a set of {\it types}, which can either be an (i) $\intType{}$, or a (ii) $\stringType{}$, or an (iii) an $\addrType{}$ of a contract or user, or a (iv) a role $\role{} \in \Roles{}$, or a (v) workflow $\workflow{} \in \Workflows{}$ (as defined next).
\item $\Workflows{}$: a set of {\it workflows}; a workflow $\workflow{} \in \Workflows{}$ is a tuple $\langle \WfStates{\workflow{}}, \WfInitState{\workflow{}}, \WfProperties{\workflow{}},  \WfInstanceProperties{\workflow{}}, \WfFunctions{\workflow{}}, \AccessControl{\workflow{}}, \accessSet{0}{\workflow{}}, \WfTransitions{\workflow{}}\rangle$:
\begin{itemize}[leftmargin=*]
\item $\WfStates{\workflow{}}$, a bounded set of states,
\item $\WfInitState{\workflow{}} \in \WfStates{\workflow{}}$, an initial state,
\item $\WfProperties{\workflow{}}$, a set of {\it properties} where a property $(\Identifier{}: \type{}) \in \WfProperties{\workflow{}}$ has a type $\type{} \in \Types{}$ and a string identifier $\Identifier{}$. 
\item A subset of properties $\WfInstanceProperties{\workflow{}} \subseteq \WfProperties{\workflow{}}$ are {\it instance roles}, where the types are roles from $\Roles{}$. 
That is, for any $(\Identifier{}: \type{}) \in \WfInstanceProperties{\workflow{}}$, $\type{}$ is a member of $\Roles{}$. 
The intuition is that a specific instance of a workflow may designate only a subset of members from a given role to execute certain action. 
The instance role variables capture such instance specific users who are members of a given role $\type{} \in \Roles{}$. 
\item A set of {\it function types} $\WfFunctions{\workflow{}}$, where each function type  $\WfFunction{}(\Identifier{0}: \type{0}, \ldots, \Identifier{k-1}: \type{k-1}) \in \WfFunctions{\workflow{}}$ consists of
\begin{itemize}
\item The function name $\WfFunction{}$, 
\item Empty list of return parameters,	
\item An arity $k \geq 0$ of the input parameters, 
\item A type $\type{i} \in \Types{}$ and an identifier $\Identifier{i}$ for the $i$-th parameter ($i \in [0, k)$), counting from zero. 
\end{itemize}
\item A {\it constructor} type $\workflow{}(\param{0}: \type{0}, \ldots, \param{k-1}: \type{k-1}) \in \WfFunctions{\workflow{}}$ where the function name equals the workflow name.
\item The {\it access control} set $\AccessControl{\workflow{}} \doteq \WfInstanceProperties{\workflow{}} \cup \Roles{}$ is a set over  the union of  the instance role properties $\WfInstanceProperties{\workflow{}}$ and the set of global roles in $\Roles{}$.  
One can restrict the invocation of a function within a transition by insisting that the $\sender{}$ belongs to a subset of $\AccessControl{\workflow{}}$. 
\item The initiator access control $\accessSet{0}{\workflow{}} \subseteq \Roles{}$ for restricting users who can create an instance of the contract by calling the constructor. 
\item Finally, a set transitions $\WfTransitions{\workflow{}} \subseteq \WfStates{\workflow{}} \times \WfFunctions{\workflow{}} \times \AccessControl{} \times 2^{\WfStates{\workflow{}}}$. 
Intuitively, a transition $(\WfState{1}, \WfFunction{}, \accessSet{}{\workflow{}}, \WfStates{2}) \in \WfTransitions{\workflow{}}$ indicates the system can transition from state $\WfState{1}$ to one of states in $\WfStates{2} \subseteq \WfStates{\workflow{}}$ (non-deterministically) by invoking the function $\WfFunction{} \in \WfFunctions{\workflow{}}$ provided the ``sender'' of $\WfFunction{}$ is a member of the access control set $\accessSet{}{\workflow{}}$. 

\end{itemize}
\end{itemize} 



\subsection{Example}
Consider the \workbenchInterface{} for the \helloBlockchain{} application described in Section~\ref{sec:overview}:
\begin{itemize}[leftmargin=*]
\item Set of global roles $\Roles{} \doteq \{\requestorRole, \ \responderRole\}$
\item Set of types $\Types{} \doteq \{\requestorRole, \responderRole \} \ \cup \ \{\intType, \stringType\} \ \cup \ \{\helloBlockchain\}$
\item A single workflow $\Workflows{} \doteq \{\helloBlockchain{}\}$ (we drop the $\workflow{}$ suffix) with:
\begin{itemize}
\item Set of workflow states $\WfStates{} \doteq \{\requestState, \ \respondState\}$,
\item The start state $\WfInitState{} \doteq \requestState$,
\item The set of properties (or fields) $\WfProperties{} \doteq \{$$\requestMessage$: $\stringType$, $\responseMessage$: $\stringType$, $\instanceRequestor$: $\requestorRole$, $\instanceResponder$: $\responderRole$$\}$.
\item The set of instance role properties are $\WfInstanceProperties{} \doteq \{$\instanceRequestor$:$\requestorRole$, $\instanceResponder$: $\responderRole$\} \subseteq \WfProperties{}$.
\item The set of 3 functions 
\begin{itemize}
\item The constructor $\helloBlockchain$($\texttt{message}$: $\stringType$),
\item Two functions $\sendRequest{}$($\texttt{requestMessage}$: $\stringType$) and $\sendResponse{}$($\texttt{responseMessage}$: $\stringType$). 
\end{itemize}
\item The access control set $\AccessControl{} \doteq \{\instanceRequestor, \instanceResponder\} \cup \{\requestorRole, \responderRole\}$, with the initiator access contorl $\accessSet{0}{} \doteq \{\requestorRole\}$.
\item Finally, there are two state-transitions in $\WfTransitions{}$ as depicted in Figure~\ref{fig:helloblockchain-fig}.
\begin{itemize}
\item $(\requestState, \sendResponse, \{\responderRole\}, \{\respondState\})$
\item $(\respondState, \sendRequest, \{\instanceRequestor\}, \{\requestState\})$
\end{itemize}
\end{itemize}
\end{itemize}




Given a \workbenchInterface{} $\Appl$ in the form of a JSON file and a smart contract $C$ (a Solidity program), we would like to ensure that the smart contract $C$ correctly implements the interface and the state transitions described in $W$.
%This is crucial to ensure that the Workbench UI state and the state of the smart contract on blockchain are synchronized; otherwise, the UI may stop responding to user requests or take the application to unexpected states.  
This is crucial to ensure that the high-level workflow specified in the application configuration file $\Appl$ by the designer is correctly implemented in the smart contract. 


We can divide this task into (a) structural and (b) semantic conformance checking. 
The structural conformance checking ensures that the data members, states and types specified in $W$ match those in $C$.
The semantic conformance checking ensures that the smart contract $C$ (that is structurally conformant with $\Appl$) correctly implements the access control and state transitions in $W$. 
Whereas the structural checking problem can be stated purely in terms of the abstract syntax tree of $C$, the semantic checks require reasoning over the dynamic runtime states of $C$.
In Section~\ref{sec:semantic-conformance}, we formalize the problem of semantic conformance by providing an axiomatic semantics over an abstract smart contract language. 
Next, we describe a program instrumentation technique for runtime enforcement of these checks, and provide a concrete implementation for Solidity based smart contracts. 
%In Section~\ref{sec:xxx}, we show how to use a static program verifier to discharge these checks at compile time. 


%% structural conformance
%\subsection{Structural Conformance}
We first state an abstract version of structural conformance checking in this Section --- the concrete details rely on the choice of language in which the smart contract is expressed (e.g. Solidity).
%
Given a \workbenchInterface{} $\Appl(\Roles{}, \Workflows{}, \Types{})$ and a smart contract $C$, the structural conformance checker enforces the following for each workflow $\workflow{} \in \Workflows{}$: 
%\begin{itemize}
%\item 
(i) There exists a contract or class named $\workflow{}$ in $C$, and the
%\item The 
the matched class for $\workflow{}$ contains
%\begin{itemize}
%\item A 
(a) a member variable named $\WfStateVar{}$ whose range is $\workflow{}.\WfStates{}$, the set of states in $\workflow{}$,
%\item A 
(b) a matching member variable or field for each $\WfProperty{} \in \workflow{}.\WfProperties{}$ with compatible types,  
%\item A 
and a matching constructor function and public functions that match the constructor and the functions in the workflow. 
Each function needs to have matching name as well as matching parameter name list, with compatible types. 
%\end{itemize}
%\end{itemize}
%Note that for the fields and functions, we do not require that the types in the smart contract are identical to the types in the workflow interface $\Appl$.
%We only need to ensure that the types are {\it compatible} (e.g. an $\intType{}$ from the interface can match with a \texttt{int16} type in the implementation). 
The Workbench system already provides one such structural conformance checker for Solidity. 


%% semantic conformance
\subsection{Semantic Conformance}
\label{sec:semantic-conformance}

In this section, we show how to ensure that a structurally conformant smart contract implements the access control and state transitions according to the \workbenchInterface{} specification.
We formalize these checks using an axiomatic semantics for a generic smart contract that supports constructors and function invocation.
We use the Floyd-Hoare triple notation for partial correctness 
\[
\begin{array}{c}
\{ \phi \} \\
c \\
\{\psi\}
\end{array}
\]

\noindent to denote that for any execution $\sigma$ of the statement $c$ from a state satisfying the predicate $\phi$, $\sigma$ does not fail any assertions and, upon termination, will end up in a state satisfying the predicate $\psi$. 
We do not require the execution to terminate however. 

Let $x$ be an instance of workflow $w$.
At a high-level, the idea is simple: we insist that when a function (respectively, the constructor) is executed along a transition (respectively, during contract creation), the resulting state transition should be in accordance with the workbench application specification.
%Moreover, the data members in the contract of {\it role} type hold addresses that only belong to the role. 

\newcommand{\isUserAddress}{{\mathit isUser}}

\begin{enumerate}[leftmargin=*]
\item {\bf Constructor}. 
We ensure that a successful termination of the constructor (of arity $k$) during the creation of an instance of the workflow by a user ($\sender$) with the appropriate access control $\accessSet{0}{\workflow{}}$ results in establishing the initial state $\WfInitState{\workflow{}}$.
\[
\begin{array}{c}
\{\neg \isUserAddress(\sender) \vee \sender \in \accessSet{0}{\workflow{}}\} \\
 x.\workflow{}(v_1, \ldots, v_{k}) \\ 
\{x.\WfStateVar{} = \WfInitState{\workflow{}}\} 
\end{array}
\]
We use a predicate $\isUserAddress$ that checks if an  address on blockchain refers to an user address or the address of a contract; the exact implementation would depend on the particular choice of language in which a smart contract is expressed. 
We weaken the access control check $\sender \in \accessSet{0}{\workflow{}}$ with the predicate $\neg \isUserAddress(\sender)$ to indicate that the access control applies only to user addresses (and not to the address of contracts). 
There are sample contracts in Workbench (e.g. \texttt{BazaarItem}~\cite{workbench-samples}) that  expect a contract instance to be only created by another contract to enforce some encapsulation, and not be created directly by an user. 
This is achieved by specifying $\accessSet{0}{\workflow{}}$ to be the empty set. 

%Second, the constructor has no terminating executions when executed with incorrect permissions for $\sender{}$. 
%$$
%\{\sender \not\in \accessSet{0}{\workflow{}}\} \ x.\workflow{}(v_1, \ldots, v_{k}) \ \{\mathit{false}\}
%$$

\item {\bf Transition Functions}. For a transition  $(\WfState{1}, \WfFunction{}, \accessSet{}{\workflow{}}, \WfStates{2}) \in \WfTransitions{\workflow{}}$ we  ensure that if $\WfFunction{}$ (with arity $k$) is invoked from the state $\WfState{1}$ of the transition by a user  in $\accessSet{}{\workflow{}}$, then the state of the smart contract instance transitions to one of the successor states in $\WfStates{2}$.

\newcommand{\emptyStack}{{\textit callStack} = []}

\[
\begin{array}{c}
\{\sender \in \accessSet{}{\workflow{}} \wedge x.\WfStateVar{} = \WfState{1}\} \\ 
 x.\WfFunction{}(v_1, \ldots, v_{k}) \\
\{x.\WfStateVar{} \in \WfStates{2}\}
\end{array}
\]

The precondition checks two facts: 
%(i) $\WfFunction{}$ is invoked with an empty call stack implying that $\WfFunction{}$ is the function invoked from a  transaction by a user address $\sender$, 
(i) the $\sender$ satisfies the access control and thus is a user address and (iii) the start state is $\WfState{1}$. 
%We add the first check to disregard nested calls to $\WfFunction{}$ that can be made from the same contract --- note that the check $\sender \in \accessSet{}{\workflow{}}$ is $\bfalse$ when the sender is another contract. 
%Although such nested calls may cause state transition in the smart contract, we only enforce the state transition checks for top-level calls to functions. 

%Second, the function $\WfAltFunction{} \in \WfFunctions{\workflow{}}$ has a terminating execution only when invoked along one of the transitions. 
%Let $\phi_{\WfAltFunction{}}$ denote the condition that captures all possible start state and access control for the sender for the transitions along which $\WfAltFunction{}$ is executed as an action. 
%Let $\WfTransitions{\workflow{}}^{\WfAltFunction{}} \doteq \{t \in \WfTransitions{\workflow{}} \ | \ t.\WfFunction{} == \WfAltFunction{} \}$ be the subset of transitions along which $\WfAltFunction{}$ is invoked. 
%$$
%\phi_{\WfAltFunction{}} \doteq \bigvee_{t \in \WfTransitions{\workflow{}}^{\WfAltFunction{}}} (\sender \in t.\accessSet{}{\workflow{}} \wedge x.\WfStateVar{} = t.\WfState{})
%$$

%When executed from any other configuration, the execution has no terminating executions. 
%$$
%\{\neg \phi_{\WfAltFunction{}}\} \ x.\WfAltFunction{}(v_1, \ldots, v_{k}) \ \{\mathit{false}\}
%$$

%Note that the Workbench infrastructure that invokes enabled functions in a state ensures that the user invokes a function only along some valid transition.
%However, a function may be executed from another contract (via an external function call), at which time the state and access control is not guaranteed by the Workbench.
%Hence, we need to put this precondition for a method to ensure that the method does not execute even in such cases.

%\item{\bf Instance Role Invariant.}
%Consider a data member $(p: r) \in \WfInstanceProperties{\workflow{}}$, where $r \in \Roles{}$ is a role type.
%We insist that whenever such an instance role field $x.p$ holds a non-zero value (i.e. other than 0x0), then it is an address that is a member of the global role $r$.
%Note that a global role (such as $\requestorRole$ in \helloBlockchain) denotes a dynamic list of addresses that can be added or removed by a Workbench application owner. 
%We assume that the null address (0x0) is not a member of any roles, as it does not represent a valid user  address. 

%We ensure that the constructor establishes the instance role invariant. 
%$$
%\{\mathit{true}\} \ \workflow{}(v_1, \ldots, v_{k}) \ \{\bigwedge_{(\Identifier{}: r) \in \WfInstanceProperties{\workflow{}}} \Identifier{} \in r \ \cup \ \{0x0\}\}
%$$
%and any function execution preserves the instance role invariant. 
%$$
%\{\bigwedge_{(\Identifier{}: r) \in \WfInstanceProperties{\workflow{}}} \Identifier{} \in r \ \cup \ \{0x0\}\} \ x.\WfFunction{}(v_1, \ldots, v_{k}) \ \{\bigwedge_{(\Identifier{}: r) \in \WfInstanceProperties{\workflow{}}} \Identifier{} \in r \ \cup \ \{0x0\}\}
%$$

%Here $r$ is interepreted as a set of addresses that have the role $r$. 

%\Shuvendu{There is still a small window where the instance role invariant can be broken and a transition function call can be made and then restored. We ignore this case to avoid instrumenting every update to the instance role variables.}
\end{enumerate}


\paragraph{\bf Type invariant.}
In addition to these two checks, one can also postulate a type invariant for any instance role variable $\Identifier{}$ of role type $r$.
One can check that whenever such an instance role variable $\Identifier{}$ holds a non-zero value (i.e. other than 0x0), then it is an address that is a member of the global role $r$; recall that a global role (such as $\requestorRole$ in \helloBlockchain) denotes a dynamic list of addresses that can be added or removed by a Workbench application owner. 
%Note that a global role (such as $\requestorRole$ in \helloBlockchain) denotes a dynamic list of addresses that can be added or removed by a Workbench application owner. 
%We assume that the null address (0x0) is not a member of any roles, as it does not represent a valid user  address. 
However, such a check ($\Identifier{} \in r \ \cup \ \{0x0\}$ ) is really a precondition that is asserted at (i) entry to any public method, and (ii) after any assignment to $\Identifier{}$ in the method body.
We think of this as a precondition since the value of this predicate depends on the contents of $r$, which can be seen as an input to a function. 
Since it does not add any runtime assertions to verify statically, we omit this check in our conformance checking.

\subsection{Semantic Conformance for Solidity}
\label{sec:solidity-instrumentation}
In this section, we provide a concrete implementation of the semantic conformance checking for smart contracts written in the popular Solidity language for the Ethereum blockchain.
We first describe a challenge in enforcing the checks related to global roles. 
%We start with providing a description of how global roles are maintained using a special $\WfRoleRegistry$ smart contract.
We then provide program instrumentation to add the conformance checks for ensuring correct initial state and state transitions.


%\subsubsection{RoleRegistry Contract}

%\begin{figure}[h!]
%\begin{lstlisting}[style=Sol,numbers=none]
%contract RoleRegistry {
%    mapping (address => 
%                   mapping (string => bool)) RoleMapping;
%    address private owner;

%    function RoleRegistry() {
%        owner = msg.sender; 
%    }
%    function HasRole(address addr, string roleName) {
%        return RoleMapping[addr][roleName];
%    }
%    function AddRole(address addr, string roleName) {
%        require (msg.sender == owner);
%        require (addr != 0x0);
%        RoleMapping[addr][roleName] = true;
%    }
%    function RemoveRole(address addr, string roleName) {
%        require (msg.sender == owner);
%        require (addr != 0x0);
%        require (HasRole[addr][roleName]);
%        RoleMapping[addr][roleName] = false;
%    }
%}
%\end{lstlisting}
%\vspace{-0.1in}
%\caption{RoleRegistry Smart Contract.}
%\label{fig:role-registry}
%\end{figure}

%Figure~\ref{fig:role-registry} describes a Solidity smart contract that is used to maintain the global roles in $\Roles{}$ for an application $\Appl(\Roles{}, \Workflows{}, \Types{})$.
%For each application instance, an instance of the $\WfRoleRegistry$ is created and deployed on the Ethereum blockchain.
%The smart contract maintains a nested dictionary (a \texttt{mapping} construct in Solidity) that maps an address $a$ and a role name $r$ to a Boolean value denoting the membership of $a$ in $r$.
%Access control for adding and removal of addresses for roles is ensured by maintaining a $\varn{owner}$ variable that is set to the sender of  the constructor; the different state changing operations such as $\texttt{AddRole}$ and $\texttt{RemoveRole}$ are guarded by a precondition (specified using Solidity keyword \texttt{require}) $\texttt{msg.sender == owner}$.
%Most of the statements are fairly standard, and insert, remove or query the dictionary for membership of an address and a role name. 

\subsubsection{Global Roles}
Although a Workbench Application configuration declares a set of global roles in $\Roles{}$, Workbench currently does not maintain the information on the blockchain.
Workbench maintains the membership of different roles in databases outside of the blockchain.
As a result, Solidity smart contracts for a Workbench application cannot refer to global role information in the body of any function. 
Validations of access control in $\AccessControl{}$ for a transition is performed by the Workbench system directly at the time a function is invoked. 
This poses an interesting dilemma for statically verifying the semantic conformance: we can either model the state of the role database in addition to the smart contract code, or we perform a conservative verification where the content of each global role is completely non-deterministic.
We adopt the latter for two reasons:
(i) First, since the smart contracts cannot refer to global roles in current Workbench, any modification to the set of global roles (e.g. adding  a user to  the $\requestorRole$ in the \helloBlockchain{} application) will never be interleaved with a transaction that executes a function in a workflow (given the deterministic execution semantics of EVM). 
(ii) Second, given that the global roles can change arbitrarily before invoking a function, one has to assume a completely non-deterministic value of the global roles for soundness. 
Therefore, we do not introduce any spurious behaviors by assuming the global roles as being completely arbitrary sets. 

\subsubsection{Program Instrumentation}
\newcommand{\solidityExpression}[1]{\parallel{#1}\parallel}

To instrument the checks we formalized in the prior section, we use the \texttt{modifier} construct from Solidity.
A modifier has syntax very similar to a function definition in Solidity with a name and list of parameters and a body that can refer to parameters and globals in scope.
The general structure of a modifier definition without any parameters (we refer users to Solidity documentation of modifiers~\cite{solidity-modifiers}) is:
\begin{lstlisting}[style=Sol,numbers=none,basicstyle=\ttfamily ]
modifier Foo() {   
   pre-statements;
   _; // placeholder
   post-statements;
}
\end{lstlisting}
where \texttt{pre-statements} and \texttt{post-statements} are Solidity statements. 
When this modifier is applied to a function \texttt{Bar}, 
\begin{lstlisting}[style=Sol,numbers=none,basicstyle=\ttfamily ]
function Bar(int x) Foo(){   
   Bar-statements;
}
\end{lstlisting}
the Solidity compiler transforms the body of \texttt{Bar} to execute \texttt{pre-statements} (respectively, \texttt{post-statements}) before (respectively, after) \texttt{Bar-statements}.
This provides a convenient way to inject code at multiple return sites from a procedure and also inject code before the execution of the constructor code (since a constructor may invoke other base class constructors implicitly). 

We now define a couple of helper predicates before describing the actual checks. 
Let us first define a Solidity predicate $\translateAC{\accessSet{}{}}$ to encode a $\sender$ to be a member of an access-control set $\accessSet{}{}$:

\newcommand{\SolidityNonDetFn}{\texttt{NonDetFunc}}

\[
\small{
\begin{array}{lll}
\translateAC{\accessSet{}{}} & \doteq & \left\{
  \begin{array}{ll}
  \mathit{false}, & \accessSet{}{} = \{\} \\
  \mathtt{msg.sender} == q, & \accessSet{}{} = \{q \in \WfInstanceProperties{\workflow{}}\} \\
  \mathtt{\SolidityNonDetFn()} & \accessSet{}{} = \{r \in \Roles{}\} \\
%  \mathtt{Roles.HasRole(msg.sender, ``r'')} & \accessSet{}{} = \{r \in \Roles{}\} \\
  \translateAC{\accessSet{1}{}} \vee \translateAC{\accessSet{2}{}} & \accessSet{}{} = \accessSet{1}{} \cup \accessSet{2}{}
  \end{array}
  \right.
\end{array}
}
\]
Here $\SolidityNonDetFn$ is a side-effect free Solidity function that returns a non-deterministic Boolean value at each invocation.
%This would be used to model a non-deterministic function that returns an arbitrary value at each invocation.
For the sake of static verification as we describe in this paper, one can declare a function without any definition. 
This allows us to model the membership check $\sender \in \accessSet{}{}$ conservatively in the absence of global roles on the blockchain.
However, this solution is not suitable for installing actual runtime checks since a truly non-deterministic function such as $\SolidityNonDetFn$ cannot be realized; we discuss the actual runtime checks in the Appendix~\ref{sec:runtime-checks}.

Next, we define a predicate for membership of a contract state in a set of states $\WfStates{} \subseteq \WfStates{\workflow{}}$ using $\translatePostStates{\WfState{}}$ as follows:
\[
\small{
\begin{array}{lll}
\translatePostStates{\WfStates{}} & \doteq & \left\{
  \begin{array}{ll}
  \mathit{false}, & \WfStates{} = \{\} \\
  \texttt{State == StateType.}\WfState{}, &  \WfStates{} = \{\WfState{} \in \WfStates{\workflow{}}\} \\
  \translatePostStates{\WfStates{1}} \vee \translatePostStates{\WfStates{2}}, & \WfStates{} = \WfStates{1} \cup \WfStates{2} \\
  \end{array}
  \right.
\end{array}
}
\]

We use these predicates to define the source code transformations below:
\begin{itemize}[leftmargin=*]
\item {\bf Constructor.} For a workflow $\workflow{}$, we add the following modifier to constructor. 

\begin{lstlisting}[style=Sol,numbers=none,basicstyle=\ttfamily \scriptsize]
modifier constructor_checker() {   
   require ($\texttt{msg.sender} \neq \texttt{tx.origin} \vee \translateAC{\accessSet{0}{\workflow{}}}$);	
   _;
   assert ($\translatePostStates{\{\WfInitState{\workflow{}}}\}$);
}
\end{lstlisting}
It is not hard to see that the assertion ensures that the constructor sets up the correct intial state.
The precondition consists of two parts. 
The first disjunct $\texttt{msg.sender} \neq \texttt{tx.origin}$ checks that the constructor is invoked by another contract and not a user (the global variable \texttt{tx.origin} tracks the user address that initiates a transaction); 
this is an implementation of the $\neg \isUserAddress(\sender)$ predicate abstractly stated in earlier section. 
The second disjunct  $\translateAC{\accessSet{0}{\workflow{}}}$ checks the access control for the \texttt{msg.sender} for the case when it is a user address. 


\item {\bf Transition Function}
For a function $\WfAltFunction{}$, let there be multiple transitions  $\WfTransitions{}^{\WfAltFunction{}} \doteq \{t \in \WfTransitions{\workflow{}} \ | \ t.\WfFunction{} == \WfAltFunction{}\}$ where $\WfAltFunction{}$ is invoked. Let $k$ be the arity of $\WfAltFunction{}$.

\begin{lstlisting}[style=Sol,numbers=none, basicstyle=\ttfamily \scriptsize]
modifier g_checker() {
   // copy old State
   StateType oldState = State;
   // copy old instance role vars
   ...
   _;
   assert $\bigwedge_{t \in \WfTransitions{}^{\WfAltFunction{}}} \left(\texttt{old}\left(\translateAC{t.\accessSet{}{\workflow{}}}  \wedge \translatePostStates{\{t.\WfState{\workflow{}}\}}\right) \Rightarrow \translatePostStates{t.\WfStates{\workflow{}}}\right)$;
}
\end{lstlisting}

%%The precondition checks that the function is executed only when it is enabled for at least one of the transitions in $\WfTransitions{}^{\WfAltFunction{}}$. 


%The predicate \texttt{msg.sender == tx.origin} ensures that the function is not invoked from a different contract.
%We maintain a ghost state variable \texttt{depth} in each contract (initialized to 0) and incremented (respectively, decremented) at method or constructor entry (respectively, exit). 
%Together, the two conjuncts allow determining if the function $\WfAltFunction{}$ is indeed the top-level function in an user transaction. 

First, we copy the $\WfStateVar{}$ variable and all of the variables in $\WfInstanceProperties{\workflow{}}$ into corresponding ``old'' copies.
Next, the assertion checks that if the function is executed in a transition $t$, then state (denoted by $\WfStateVar{}$) transitions to one of the successor states  in $t.\WfStates{}$.
The notation $\texttt{old}(e)$ replaces any occurrences of a state variable (such as $\WfStateVar{}$) with the ``old'' copy that holds the value at entry to the function; this is required since the value of the state variables can change during the execution of the procedure.
Finally, since conjunction distributes over assertions, we can replace the single assertion with an assertion for each transition in the implementation. 

%We can perform several optimizatoins for specific cases:
%First, since conjunction distributes over assertions, we can replace the single assertion with an assertion for each transition. 
%Second, when the function $\WfAltFunction{}$ appears in exactly one transition, then we can simplify the assertion to  $\translatePostStates{t.\WfStates{\workflow{}}}$, since the premise $\texttt{old}(\translateAC{t.\accessSet{}{\workflow{}}} \ \wedge \ \translatePostStates{\{t.\WfState{\workflow{}}}\})$ is present as precondition of the modifier;
%in such a case, we can omit copying the old state of variables into temporary local variables. 

%\item {\bf Instance Role  Invariant}
%We also develop another modifier $\texttt{TypeInvariant()}$ to preserve the invariant that the instance role variables hold addresses of the corresponding roles only (unless 0x0). 

%\begin{lstlisting}[style=Sol,numbers=none, basicstyle=\ttfamily \scriptsize]
%modifier TypeInvariant() {   
%   require ($\bigwedge_{(\Identifier{}: r) \in \WfInstanceProperties{\workflow{}}}$ Roles.IsNullOrHasRole($\Identifier{}, ''r''$));
%   _;
%   assert ($\bigwedge_{(\Identifier{}: r) \in \WfInstanceProperties{\workflow{}}}$ Roles.IsNullOrHasRole($\Identifier{}, ''r''$));
%}
%\end{lstlisting}
\end{itemize}

\subsubsection{Instrumented Running Example}
Figure~\ref{fig:instrumented-running-example} shows the modifier definitions for our running example \helloBlockchain{}  described in Section~\ref{sec:overview}.
The modifiers are applied to the user-written smart contract in Figure~\ref{fig:helloblockchain-smart-contract}, and shown by the \underline{\texttt{underlined}} statements.  
We add a comment for the lines where a reference to a global role in the specification is replaced by a call to the non-deterministic function $\SolidityNonDetFn$.
%%Although one can simplify the assertions and remove the ``old'' variables (such as $\texttt{oldState}$ and $\texttt{oldRequestor}$) since the functions appear in exactly one transitions, we have retained them to show the actual assertions with the old variables. 

\begin{figure}[htbp]
\begin{lstlisting}[style=Sol,numbers=none]
   function NonDetFunc() returns (bool); //no definition  

    // Checker modifiers 
    modifier constructor_checker() 
    {
      require (msg.sender != tx.origin || 
               NonDetFunc()); // global role REQUESTOR
       _;      
      assert (State == StateType.Request);
    }
    modifier SendRequest_checker() 
    {
      StateType oldState = State;
      address oldRequestor = Requestor;
       _;
      assert ((msg.sender == oldRequestor && 
               oldState == StateType.Respond) 
              ==> State == StateType.Request);
    }
    modifier SendResponse_checker() 
    {
      StateType oldState = State;
       _;
      assert ((NonDetFunc() && // global role RESPONDER
               oldState == StateType.Request) 
              ==> State == StateType.Respond);
    }

\end{lstlisting}
\vspace{-0.1in}
\caption{Modifier definitions for instrumented HelloBlockchain application.}
\label{fig:instrumented-running-example}
\end{figure}

%\begin{theorem}
%(Assuming no other assertion in the program), the instrumented smart contract program fails an assertion if and only if one of the Hoare-triples 
%Moreover, the instrumented program also satisfies the {\it enabled-along-transitions} Hoare-triples. 
%\end{theorem}

%We will need an operational semantics for Solidity to do this proof. We will do the proof for  a smaller subset that we formalize. 

%Also, we have to show that exceptions/assertions cannot be caught. 




